Measurements of branching fractions and direct ${\it CP}$-violating asymmetries in $B^+ \to K^+ \pi^0~\mbox{and}~\pi^+ \pi^0$ decays using 2019 and 2020 Belle II data

We report measurements of branching fractions ($\mathcal B$) and direct ${\it CP}$-violating asymmetries ($\mathcal A_{\it CP}$) for the decays $B^+\to K^+\pi^0$ and $B^+ \to \pi^+\pi^0$ reconstructed with the Belle II detector in a sample of asymmetric-energy electron-positron collisions at the $\Upsilon(4S)$ resonance corresponding to 62.8 $\text{fb}^{-1}$ of integrated luminosity. The results are $\mathcal{B}(B^+ \to K^+\pi^0) = [11.9 ^{+1.1}_{-1.0} (\rm stat)\pm 1.6(\rm syst)]\times 10^{-6}$, $\mathcal{B}(B^+ \to \pi^+\pi^0) = [5.5 ^{+1.0}_{-0.9} (\rm stat)\pm 0.7(\rm syst)]\times 10^{-6}$, $\mathcal A_{\it CP}(B^+ \to K^+\pi^0) = -0.09 \pm 0.09 (\rm stat)\pm 0.03(\rm syst)$, and $\mathcal A_{\it CP}(B^+ \to \pi^+\pi^0) = -0.04 \pm 0.17 (\rm stat)\pm 0.06(\rm syst)$. The results are consistent with previous measurements and show a detector performance comparable with early Belle performance.

==> acknowledgements.tex <==
\section*{Acknowledgments}

%\input acknowledgements.tex
We thank the SuperKEKB group for the excellent operation of the
accelerator; the KEK cryogenics group for the efficient
operation of the solenoid; and the KEK computer group for
on-site computing support.
This work was supported by the following funding sources:
%Armenia
Science Committee of the Republic of Armenia Grant No. 18T-1C180;
%Australia
Australian Research Council and research grant Nos.
DP180102629, 
DP170102389, 
DP170102204, 
DP150103061, 
FT130100303, 
and
FT130100018; 
%Austria
Austrian Federal Ministry of Education, Science and Research, and
Austrian Science Fund No. P 31361-N36; 
%Canada
Natural Sciences and Engineering Research Council of Canada, Compute Canada and CANARIE;
%China
Chinese Academy of Sciences and research grant No. QYZDJ-SSW-SLH011,
National Natural Science Foundation of China and research grant Nos.
11521505,
11575017,
11675166,
11761141009,
11705209,
and
11975076,
LiaoNing Revitalization Talents Program under contract No. XLYC1807135,
Shanghai Municipal Science and Technology Committee under contract No. 19ZR1403000,
Shanghai Pujiang Program under Grant No. 18PJ1401000,
and the CAS Center for Excellence in Particle Physics (CCEPP);
%Czech Republic
the Ministry of Education, Youth and Sports of the Czech Republic under Contract No.~LTT17020 and 
Charles University grants SVV 260448 and GAUK 404316;
%EU
European Research Council, 7th Framework PIEF-GA-2013-622527, 
Horizon 2020 Marie Sklodowska-Curie grant agreement No. 700525 `NIOBE,' 
and
Horizon 2020 Marie Sklodowska-Curie RISE project JENNIFER2 grant agreement No. 822070 (European grants);
%France
L'Institut National de Physique Nucl\'{e}aire et de Physique des Particules (IN2P3) du CNRS (France);
%Germany
BMBF, DFG, HGF, MPG, AvH Foundation, and Deutsche Forschungsgemeinschaft (DFG) under Germany's Excellence Strategy -- EXC2121 ``Quantum Universe''' -- 390833306 (Germany);
%India
Department of Atomic Energy and Department of Science and Technology (India);
%Israel
Israel Science Foundation grant No. 2476/17
and
United States-Israel Binational Science Foundation grant No. 2016113;
%Italy
Istituto Nazionale di Fisica Nucleare and the research grants BELLE2;
%Japan
Japan Society for the Promotion of Science,  Grant-in-Aid for Scientific Research grant Nos.
16H03968, 
16H03993, 
16H06492,
16K05323, 
17H01133, 
17H05405, 
18K03621, 
18H03710, 
18H05226,
19H00682, % Niigata
26220706,
and
26400255,
the National Institute of Informatics, and Science Information NETwork 5 (SINET5), 
and
the Ministry of Education, Culture, Sports, Science, and Technology (MEXT) of Japan;  
%Korea
National Research Foundation (NRF) of Korea Grant Nos.
2016R1\-D1A1B\-01010135,
2016R1\-D1A1B\-02012900,
2018R1\-A2B\-3003643,
2018R1\-A6A1A\-06024970,
2018R1\-D1A1B\-07047294,
2019K1\-A3A7A\-09033840,
and
2019R1\-I1A3A\-01058933,
Radiation Science Research Institute,
Foreign Large-size Research Facility Application Supporting project,
the Global Science Experimental Data Hub Center of the Korea Institute of Science and Technology Information
and
KREONET/GLORIAD;
%Malaysia
Universiti Malaya RU grant, Akademi Sains Malaysia and Ministry of Education Malaysia;
%Mexico
% CINVESTAV-IPN, UNAM, UAS, BUAP and CONACYT are funded under
Frontiers of Science Program contracts
FOINS-296,
CB-221329,
CB-236394,
CB-254409,
and
CB-180023, and SEP-CINVESTAV research grant 237 (Mexico);
%Poland
the Polish Ministry of Science and Higher Education and the National Science Center;
%Russia
the Ministry of Science and Higher Education of the Russian Federation,
Agreement 14.W03.31.0026;
%Saudi Arabia
University of Tabuk research grants
S-1440-0321, S-0256-1438, and S-0280-1439 (Saudi Arabia);
%Slovenia
Slovenian Research Agency and research grant Nos.
J1-9124
and
P1-0135; 
%Spain
Agencia Estatal de Investigacion, Spain grant Nos.
FPA2014-55613-P
and
FPA2017-84445-P,
and
CIDEGENT/2018/020 of Generalitat Valenciana;
%Taiwan
Ministry of Science and Technology and research grant Nos.
MOST106-2112-M-002-005-MY3
and
MOST107-2119-M-002-035-MY3, 
and the Ministry of Education (Taiwan);
%Thailand
Thailand Center of Excellence in Physics;
%Turkey
TUBITAK ULAKBIM (Turkey);
%Ukraine
Ministry of Education and Science of Ukraine;
%USA
the US National Science Foundation and research grant Nos.
PHY-1807007 % Luther
and
PHY-1913789, % Indiana CEEM
and the US Department of Energy and research grant Nos.
DE-AC06-76RLO1830, % PNNL
DE{}-SC0007983, % Wayne State
DE{}-SC0009824, % Florida
DE{}-SC0009973, % VPI
DE{}-SC0010073, % South Carolina
DE{}-SC0010118, % Carnegie Mellon
DE{}-SC0010504, % Hawaii
DE{}-SC0011784, % Cincinnati
DE{}-SC0012704; % BNL
%last group
and
%Vietnam
the National Foundation for Science and Technology Development (NAFOSTED) 
of Vietnam under contract No 103.99-2018.45.

==> authors-conf2020.tex <==
%%% Paper:    (2020  conference papers)
%%% Journal:  (2020 conferences)
%%% ====================================================================
%%% Use \input{authors-conf2020} to insert this material into your latex file.
\newcommand{\instSinica}{Academia Sinica, Taipei 11529, Taiwan}
\newcommand{\instCPPM}{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\newcommand{\instBeihang}{Beihang University, Beijing 100191, China}
\newcommand{\instBUAP}{Benemerita Universidad Autonoma de Puebla, Puebla 72570, Mexico}
\newcommand{\instBNL}{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\newcommand{\instBINP}{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
\newcommand{\instCMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\newcommand{\instCinvestavIPN}{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\newcommand{\instPrague}{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\newcommand{\instChiangMai}{Chiang Mai University, Chiang Mai 50202, Thailand}
\newcommand{\instChiba}{Chiba University, Chiba 263-8522, Japan}
\newcommand{\instChonnam}{Chonnam National University, Gwangju 61186, South Korea}
\newcommand{\instConacyt}{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\newcommand{\instDESY}{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\newcommand{\instDuke}{Duke University, Durham, North Carolina 27708, U.S.A.}
\newcommand{\instITAR}{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
\newcommand{\instENEA}{ENEA Casaccia, I-00123 Roma, Italy}
\newcommand{\instEri}{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\newcommand{\instJuelich}{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich, Germany}
\newcommand{\instFuJen}{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\newcommand{\instFudan}{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\newcommand{\instGoettingen}{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
\newcommand{\instGifu}{Gifu University, Gifu 501-1193, Japan}
\newcommand{\instSOKENDAI}{The Graduate University for Advanced Studies (SOKENDAI), Hayama 240-0193, Japan}
\newcommand{\instGyeongsang}{Gyeongsang National University, Jinju 52828, South Korea}
\newcommand{\instHanyang}{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
\newcommand{\instKEK}{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instJPARC}{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instHSE}{Higher School of Economics (HSE), Moscow 101000, Russian Federation}
\newcommand{\instIISER}{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\newcommand{\instIITBhubaneswar}{Indian Institute of Technology Bhubaneswar, Satya Nagar 751007, India}
\newcommand{\instIITGuwahati}{Indian Institute of Technology Guwahati, Assam 781039, India}
\newcommand{\instIITHyderabad}{Indian Institute of Technology Hyderabad, Telangana 502285, India}
\newcommand{\instIITMadras}{Indian Institute of Technology Madras, Chennai 600036, India}
\newcommand{\instIndiana}{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\newcommand{\instIHEPRussia}{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\newcommand{\instHEPHYVienna}{Institute of High Energy Physics, Vienna 1050, Austria}
\newcommand{\instIHEPChina}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\newcommand{\instChennai}{Institute of Mathematical Sciences, Chennai 600113, India}
\newcommand{\instIPP}{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\newcommand{\instIOP}{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\newcommand{\instIFIC}{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\newcommand{\instFrascati}{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\newcommand{\instNapoliINFN}{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\newcommand{\instPadovaINFN}{INFN Sezione di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaINFN}{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaINFN}{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaINFN}{INFN Sezione di Roma, I-00185 Roma, Italy}
\newcommand{\instRomaTreINFN}{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoINFN}{INFN Sezione di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteINFN}{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\newcommand{\instJAEA}{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
\newcommand{\instMainz}{Johannes Gutenberg-Universit\"{a}t Mainz, Institut f\"{u}r Kernphysik, D-55099 Mainz, Germany}
\newcommand{\instGiessen}{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\newcommand{\instKarlsruhe}{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
\newcommand{\instKennesaw}{Kennesaw State University, Kennesaw, Georgia 30144, U.S.A.}
\newcommand{\instKitasato}{Kitasato University, Sagamihara 252-0373, Japan}
\newcommand{\instKISTI}{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\newcommand{\instKorea}{Korea University, Seoul 02841, South Korea}
\newcommand{\instKSU}{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\newcommand{\instKyotoU}{Kyoto University, Kyoto 606-8501, Japan}
\newcommand{\instKyungpook}{Kyungpook National University, Daegu 41566, South Korea}
\newcommand{\instLPI}{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991, Russian Federation}
\newcommand{\instLNNU}{Liaoning Normal University, Dalian 116029, China}
\newcommand{\instLMU}{Ludwig Maximilians University, 80539 Munich, Germany}
\newcommand{\instISUni}{Iowa State University,  Ames, Iowa 50011, U.S.A.}
\newcommand{\instLuther}{Luther College, Decorah, Iowa 52101, U.S.A.}
\newcommand{\instMNITJaipur}{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\newcommand{\instMPP}{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
\newcommand{\instMPGHLL}{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
\newcommand{\instMcGill}{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
\newcommand{\instMETU}{Middle East Technical University, 06531 Ankara, Turkey}
\newcommand{\instMEPhI}{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\newcommand{\instNagoya}{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaKMI}{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaIAR}{Institute for Advanced Research, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNaraWu}{Nara Women's University, Nara 630-8506, Japan}
\newcommand{\instUNAM}{National Autonomous University of Mexico, Mexico City, Mexico}
\newcommand{\instNTUTaiwan}{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
\newcommand{\instNUUTaiwan}{National United University, Miao Li 36003, Taiwan}
\newcommand{\instKrakow}{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\newcommand{\instNiigata}{Niigata University, Niigata 950-2181, Japan}
\newcommand{\instNSU}{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\newcommand{\instOkinawa}{Okinawa Institute of Science and Technology, Okinawa 904-0495, Japan}
\newcommand{\instOsakaCity}{Osaka City University, Osaka 558-8585, Japan}
\newcommand{\instRCNP}{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\newcommand{\instPNNL}{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\newcommand{\instPanjab}{Panjab University, Chandigarh 160014, India}
\newcommand{\instPeking}{Peking University, Beijing 100871, China}
\newcommand{\instPanjabPAU}{Punjab Agricultural University, Ludhiana 141004, India}
\newcommand{\instRIKENMSL}{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
\newcommand{\instRIKEN}{Theoretical Research Division, Nishina Center, RIKEN, Saitama 351-0198, Japan}
\newcommand{\instXavier}{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\newcommand{\instSeoul}{Seoul National University, Seoul 08826, South Korea}
\newcommand{\instShandong}{Shandong University, Jinan 250100, China}
\newcommand{\instSPU}{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\newcommand{\instSoochow}{Soochow University, Suzhou 215006, China}
\newcommand{\instSoongsil}{Soongsil University, Seoul 06978, South Korea}
\newcommand{\instLjubljanaJSI}{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\newcommand{\instKyiv}{Taras Shevchenko National Univ. of Kiev, Kiev, Ukraine}
\newcommand{\instTata}{Tata Institute of Fundamental Research, Mumbai 400005, India}
\newcommand{\instTUM}{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\newcommand{\instECUTUM}{Excellence Cluster Universe, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\newcommand{\instTelAviv}{Tel Aviv University, School of Physics and Astronomy, Tel Aviv, 69978, Israel}
\newcommand{\instToho}{Toho University, Funabashi 274-8510, Japan}
\newcommand{\instTohoku}{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
\newcommand{\instTitech}{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
\newcommand{\instTokyoMetropolitan}{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\newcommand{\instUAS}{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
\newcommand{\instNapoliUNIV}{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\newcommand{\instNapoliUNIVA}{Dipartimento di Agraria, Universit\`{a} di Napoli Federico II, I-80055 Portici (NA), Italy}
\newcommand{\instPadovaUNIV}{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaUNIV}{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaUNIV}{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaUNIV}{Universit\`{a} di Roma ``La Sapienza,'' I-00185 Roma, Italy}
\newcommand{\instRomaTreUNIV}{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoUNIV}{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteUNIV}{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
\newcommand{\instMontreal}{Universit\'{e} de Montr\'{e}al, Physique des Particules, Montr\'{e}al, Qu\'{e}bec, H3C 3J7, Canada}
\newcommand{\instIJCLab}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\newcommand{\instIPHC}{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\newcommand{\instAdelaide}{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
\newcommand{\instBonn}{University of Bonn, 53115 Bonn, Germany}
\newcommand{\instUBC}{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\newcommand{\instCincinnati}{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\newcommand{\instFlorida}{University of Florida, Gainesville, Florida 32611, U.S.A.}
\newcommand{\instHamburg}{University of Hamburg, 20148 Hamburg, Germany}
\newcommand{\instHawaii}{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\newcommand{\instHeidelberg}{University of Heidelberg, 68131 Mannheim, Germany}
\newcommand{\instLjubljanaUniLJ}{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\newcommand{\instLouisville}{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
\newcommand{\instMalaya}{National Centre for Particle Physics, University Malaya, 50603 Kuala Lumpur, Malaysia}
\newcommand{\instLjubljanaUM}{University of Maribor, 2000 Maribor, Slovenia}
\newcommand{\instMelbourne}{School of Physics, University of Melbourne, Victoria 3010, Australia}
\newcommand{\instMississippi}{University of Mississippi, University, Mississippi 38677, U.S.A.}
\newcommand{\instUOM}{University of Miyazaki, Miyazaki 889-2192, Japan}
\newcommand{\instNovaGorica}{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\newcommand{\instPittsburgh}{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\newcommand{\instUSTC}{University of Science and Technology of China, Hefei 230026, China}
\newcommand{\instSAlabama}{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
\newcommand{\instSCarolina}{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\newcommand{\instSydney}{School of Physics, University of Sydney, New South Wales 2006, Australia}
\newcommand{\instTabuk}{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\newcommand{\instUTokyo}{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\newcommand{\instIPMU}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\newcommand{\instVictoria}{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\newcommand{\instVPI}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\newcommand{\instWayneState}{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\newcommand{\instYamagata}{Yamagata University, Yamagata 990-8560, Japan}
\newcommand{\instYerevan}{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
\newcommand{\instYonsei}{Yonsei University, Seoul 03722, South Korea}
%%%\affiliation{\instSinica}
\affiliation{\instCPPM}
\affiliation{\instBeihang}
%%%\affiliation{\instBUAP}
\affiliation{\instBNL}
\affiliation{\instBINP}
\affiliation{\instCMU}
\affiliation{\instCinvestavIPN}
\affiliation{\instPrague}
\affiliation{\instChiangMai}
\affiliation{\instChiba}
\affiliation{\instChonnam}
\affiliation{\instConacyt}
\affiliation{\instDESY}
\affiliation{\instDuke}
\affiliation{\instITAR}
%%%\affiliation{\instENEA}
\affiliation{\instEri}
\affiliation{\instJuelich}
\affiliation{\instFuJen}
\affiliation{\instFudan}
\affiliation{\instGoettingen}
\affiliation{\instGifu}
\affiliation{\instSOKENDAI}
\affiliation{\instGyeongsang}
\affiliation{\instHanyang}
\affiliation{\instKEK}
\affiliation{\instJPARC}
\affiliation{\instHSE}
\affiliation{\instIISER}
\affiliation{\instIITBhubaneswar}
\affiliation{\instIITGuwahati}
\affiliation{\instIITHyderabad}
\affiliation{\instIITMadras}
\affiliation{\instIndiana}
\affiliation{\instIHEPRussia}
\affiliation{\instHEPHYVienna}
\affiliation{\instIHEPChina}
%%%\affiliation{\instChennai}
\affiliation{\instIPP}
\affiliation{\instIOP}
\affiliation{\instIFIC}
\affiliation{\instFrascati}
\affiliation{\instNapoliINFN}
\affiliation{\instPadovaINFN}
\affiliation{\instPerugiaINFN}
\affiliation{\instPisaINFN}
\affiliation{\instRomaINFN}
\affiliation{\instRomaTreINFN}
\affiliation{\instTorinoINFN}
\affiliation{\instTriesteINFN}
\affiliation{\instISUni}
\affiliation{\instJAEA}
\affiliation{\instMainz}
\affiliation{\instGiessen}
\affiliation{\instKarlsruhe}
%%%\affiliation{\instKennesaw}
\affiliation{\instKitasato}
\affiliation{\instKISTI}
\affiliation{\instKorea}
\affiliation{\instKSU}
%%%\affiliation{\instKyotoU}
\affiliation{\instKyungpook}
\affiliation{\instLPI}
\affiliation{\instLNNU}
\affiliation{\instLMU}
\affiliation{\instLuther}
\affiliation{\instMNITJaipur}
\affiliation{\instMPP}
\affiliation{\instMPGHLL}
\affiliation{\instMcGill}
%%%\affiliation{\instMETU}
\affiliation{\instMEPhI}
\affiliation{\instNagoya}
\affiliation{\instNagoyaKMI}
\affiliation{\instNagoyaIAR}
\affiliation{\instNaraWu}
%%%\affiliation{\instUNAM}
\affiliation{\instNTUTaiwan}
\affiliation{\instNUUTaiwan}
\affiliation{\instKrakow}
\affiliation{\instNiigata}
\affiliation{\instNSU}
\affiliation{\instOkinawa}
\affiliation{\instOsakaCity}
\affiliation{\instRCNP}
\affiliation{\instPNNL}
\affiliation{\instPanjab}
\affiliation{\instPeking}
\affiliation{\instPanjabPAU}
\affiliation{\instRIKENMSL}
%%%\affiliation{\instRIKEN}
%%%\affiliation{\instXavier}
\affiliation{\instSeoul}
%%%\affiliation{\instShandong}
\affiliation{\instSPU}
\affiliation{\instSoochow}
\affiliation{\instSoongsil}
\affiliation{\instLjubljanaJSI}
\affiliation{\instKyiv}
\affiliation{\instTata}
\affiliation{\instTUM}
%%%\affiliation{\instECUTUM}
\affiliation{\instTelAviv}
\affiliation{\instToho}
\affiliation{\instTohoku}
\affiliation{\instTitech}
\affiliation{\instTokyoMetropolitan}
\affiliation{\instUAS}
\affiliation{\instNapoliUNIV}
\affiliation{\instPadovaUNIV}
\affiliation{\instPerugiaUNIV}
\affiliation{\instPisaUNIV}
\affiliation{\instRomaUNIV}
\affiliation{\instRomaTreUNIV}
\affiliation{\instTorinoUNIV}
\affiliation{\instTriesteUNIV}
\affiliation{\instMontreal}
\affiliation{\instIJCLab}
\affiliation{\instIPHC}
\affiliation{\instAdelaide}
\affiliation{\instBonn}
\affiliation{\instUBC}
\affiliation{\instCincinnati}
\affiliation{\instFlorida}
%%%\affiliation{\instHamburg}
\affiliation{\instHawaii}
\affiliation{\instHeidelberg}
\affiliation{\instLjubljanaUniLJ}
\affiliation{\instLouisville}
\affiliation{\instMalaya}
\affiliation{\instLjubljanaUM}
\affiliation{\instMelbourne}
\affiliation{\instMississippi}
\affiliation{\instUOM}
%%%\affiliation{\instNovaGorica}
\affiliation{\instPittsburgh}
\affiliation{\instUSTC}
\affiliation{\instSAlabama}
\affiliation{\instSCarolina}
\affiliation{\instSydney}
%%%\affiliation{\instTabuk}
\affiliation{\instUTokyo}
\affiliation{\instIPMU}
\affiliation{\instVictoria}
\affiliation{\instVPI}
\affiliation{\instWayneState}
\affiliation{\instYamagata}
\affiliation{\instYerevan}
\affiliation{\instYonsei}
  \author{F.~Abudin{\'e}n}\affiliation{\instTriesteINFN} % 2250
  \author{I.~Adachi}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2590
  \author{R.~Adak}\affiliation{\instFudan} % 6743
  \author{K.~Adamczyk}\affiliation{\instKrakow} % 2239
  \author{P.~Ahlburg}\affiliation{\instBonn} % 2367
  \author{J.~K.~Ahn}\affiliation{\instKorea} % 7423
  \author{H.~Aihara}\affiliation{\instUTokyo} % 2223
  \author{N.~Akopov}\affiliation{\instYerevan} % 9443
  \author{A.~Aloisio}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2194
  \author{F.~Ameli}\affiliation{\instRomaINFN} % 4683
  \author{L.~Andricek}\affiliation{\instMPGHLL} % 2098
  \author{N.~Anh~Ky}\affiliation{\instIOP}\affiliation{\instITAR} % 2218
  \author{D.~M.~Asner}\affiliation{\instBNL} % 4684
  \author{H.~Atmacan}\affiliation{\instCincinnati} % 2538
  \author{V.~Aulchenko}\affiliation{\instBINP}\affiliation{\instNSU} % 8183
  \author{T.~Aushev}\affiliation{\instHSE} % 3747
  \author{V.~Aushev}\affiliation{\instKyiv} % 2155
  \author{T.~Aziz}\affiliation{\instTata} % 3523
  \author{V.~Babu}\affiliation{\instDESY} % 5623
  \author{S.~Bacher}\affiliation{\instKrakow} % 2258
  \author{S.~Baehr}\affiliation{\instKarlsruhe} % 2515
  \author{S.~Bahinipati}\affiliation{\instIITBhubaneswar} % 2332
  \author{A.~M.~Bakich}\affiliation{\instSydney} % 2115
  \author{P.~Bambade}\affiliation{\instIJCLab} % 3003
  \author{Sw.~Banerjee}\affiliation{\instLouisville} % 8603
  \author{S.~Bansal}\affiliation{\instPanjab} % 5163
  \author{M.~Barrett}\affiliation{\instKEK} % 2180
  \author{G.~Batignani}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 6643
  \author{J.~Baudot}\affiliation{\instIPHC} % 2562
  \author{A.~Beaulieu}\affiliation{\instVictoria} % 2444
  \author{J.~Becker}\affiliation{\instKarlsruhe} % 5403
  \author{P.~K.~Behera}\affiliation{\instIITMadras} % 4204
  \author{M.~Bender}\affiliation{\instLMU} % 2440
  \author{J.~V.~Bennett}\affiliation{\instMississippi} % 2454
  \author{E.~Bernieri}\affiliation{\instRomaTreINFN} % 4483
  \author{F.~U.~Bernlochner}\affiliation{\instBonn} % 2282
  \author{M.~Bertemes}\affiliation{\instHEPHYVienna} % 2595
  \author{M.~Bessner}\affiliation{\instHawaii} % 3783
  \author{S.~Bettarini}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2350
  \author{V.~Bhardwaj}\affiliation{\instIISER} % 2228
  \author{B.~Bhuyan}\affiliation{\instIITGuwahati} % 2097
  \author{F.~Bianchi}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2564
  \author{T.~Bilka}\affiliation{\instPrague} % 2484
  \author{S.~Bilokin}\affiliation{\instLMU} % 3623
  \author{D.~Biswas}\affiliation{\instLouisville} % 8703
  \author{A.~Bobrov}\affiliation{\instBINP}\affiliation{\instNSU} % 2294
  \author{A.~Bondar}\affiliation{\instBINP}\affiliation{\instNSU} % 4643
  \author{G.~Bonvicini}\affiliation{\instWayneState} % 2095
  \author{A.~Bozek}\affiliation{\instKrakow} % 2303
  \author{M.~Bra\v{c}ko}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % 2425
  \author{P.~Branchini}\affiliation{\instRomaTreINFN} % 2577
  \author{N.~Braun}\affiliation{\instKarlsruhe} % 2436
  \author{R.~A.~Briere}\affiliation{\instCMU} % 2584
  \author{T.~E.~Browder}\affiliation{\instHawaii} % 2560
  \author{D.~N.~Brown}\affiliation{\instLouisville} % 8743
  \author{A.~Budano}\affiliation{\instRomaTreINFN} % 2171
  \author{L.~Burmistrov}\affiliation{\instIJCLab} % 2111
  \author{S.~Bussino}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 5384
  \author{M.~Campajola}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 5223
  \author{L.~Cao}\affiliation{\instBonn} % 2099
  \author{G.~Caria}\affiliation{\instMelbourne} % 2438
  \author{G.~Casarosa}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2491
  \author{C.~Cecchi}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 2433
  \author{D.~\v{C}ervenkov}\affiliation{\instPrague} % 2078
  \author{M.-C.~Chang}\affiliation{\instFuJen} % 2827
  \author{P.~Chang}\affiliation{\instNTUTaiwan} % 2542
  \author{R.~Cheaib}\affiliation{\instUBC} % 2208
  \author{V.~Chekelian}\affiliation{\instMPP} % 2167
  \author{C.~Chen}\affiliation{\instISUni}
\author{Y.-C.~Chen}\affiliation{\instNTUTaiwan} % 
  \author{Y.~Q.~Chen}\affiliation{\instUSTC} % 2576
  \author{Y.-T.~Chen}\affiliation{\instNTUTaiwan} % 2884
  \author{B.~G.~Cheon}\affiliation{\instHanyang} % 2173
  \author{K.~Chilikin}\affiliation{\instLPI} % 2308
  \author{K.~Chirapatpimol}\affiliation{\instChiangMai} % 10803
  \author{H.-E.~Cho}\affiliation{\instHanyang} % 2182
  \author{K.~Cho}\affiliation{\instKISTI} % 2516
  \author{S.-J.~Cho}\affiliation{\instYonsei} % 2723
  \author{S.-K.~Choi}\affiliation{\instGyeongsang} % 2364
  \author{S.~Choudhury}\affiliation{\instIITHyderabad} % 2206
  \author{D.~Cinabro}\affiliation{\instWayneState} % 2092
  \author{L.~Corona}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 3944
  \author{L.~M.~Cremaldi}\affiliation{\instMississippi} % 2276
  \author{D.~Cuesta}\affiliation{\instIPHC} % 2668
  \author{S.~Cunliffe}\affiliation{\instDESY} % 2272
  \author{T.~Czank}\affiliation{\instIPMU} % 2254
  \author{N.~Dash}\affiliation{\instIITMadras} % 2601
  \author{F.~Dattola}\affiliation{\instDESY} % 3745
  \author{E.~De~La~Cruz-Burelo}\affiliation{\instCinvestavIPN} % 2359
  \author{G.~De~Nardo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2459
  \author{M.~De~Nuccio}\affiliation{\instDESY} % 2610
  \author{G.~De~Pietro}\affiliation{\instRomaTreINFN} % 2528
  \author{R.~de~Sangro}\affiliation{\instFrascati} % 2524
  \author{B.~Deschamps}\affiliation{\instBonn} % 2671
  \author{M.~Destefanis}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2594
  \author{S.~Dey}\affiliation{\instTelAviv} % 5023
  \author{A.~De~Yta-Hernandez}\affiliation{\instCinvestavIPN} % 2104
  \author{A.~Di~Canto}\affiliation{\instBNL} % 10963
  \author{F.~Di~Capua}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2065
  \author{S.~Di~Carlo}\affiliation{\instIJCLab} % 2079
  \author{J.~Dingfelder}\affiliation{\instBonn} % 2151
  \author{Z.~Dole\v{z}al}\affiliation{\instPrague} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez}\affiliation{\instUAS} % 2191
  \author{T.~V.~Dong}\affiliation{\instFudan} % 2215
  \author{K.~Dort}\affiliation{\instGiessen} % 5583
  \author{D.~Dossett}\affiliation{\instMelbourne} % 2574
  \author{S.~Dubey}\affiliation{\instHawaii} % 11063
  \author{S.~Duell}\affiliation{\instBonn} % 2344
  \author{G.~Dujany}\affiliation{\instIPHC} % 9703
  \author{S.~Eidelman}\affiliation{\instBINP}\affiliation{\instLPI}\affiliation{\instNSU} % 4984
  \author{M.~Eliachevitch}\affiliation{\instBonn} % 2725
  \author{D.~Epifanov}\affiliation{\instBINP}\affiliation{\instNSU} % 2551
  \author{J.~E.~Fast}\affiliation{\instPNNL} % 2264
  \author{T.~Ferber}\affiliation{\instDESY} % 2482
  \author{D.~Ferlewicz}\affiliation{\instMelbourne} % 2073
  \author{G.~Finocchiaro}\affiliation{\instFrascati} % 2400
  \author{S.~Fiore}\affiliation{\instRomaINFN} % 4225
  \author{P.~Fischer}\affiliation{\instHeidelberg} % 2141
  \author{A.~Fodor}\affiliation{\instMcGill} % 2312
  \author{F.~Forti}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2432
  \author{A.~Frey}\affiliation{\instGoettingen} % 2150
  \author{M.~Friedl}\affiliation{\instHEPHYVienna} % 2442
  \author{B.~G.~Fulsom}\affiliation{\instPNNL} % 2563
  \author{M.~Gabriel}\affiliation{\instMPP} % 2443
  \author{N.~Gabyshev}\affiliation{\instBINP}\affiliation{\instNSU} % 2510
  \author{E.~Ganiev}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 4623
  \author{M.~Garcia-Hernandez}\affiliation{\instCinvestavIPN} % 4823
  \author{R.~Garg}\affiliation{\instPanjab} % 2213
  \author{A.~Garmash}\affiliation{\instBINP}\affiliation{\instNSU} % 2161
  \author{V.~Gaur}\affiliation{\instVPI} % 2413
  \author{A.~Gaz}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2181
  \author{U.~Gebauer}\affiliation{\instGoettingen} % 2174
  \author{M.~Gelb}\affiliation{\instKarlsruhe} % 2340
  \author{A.~Gellrich}\affiliation{\instDESY} % 2480
  \author{J.~Gemmler}\affiliation{\instKarlsruhe} % 2321
  \author{T.~Ge{\ss}ler}\affiliation{\instGiessen} % 2121
  \author{D.~Getzkow}\affiliation{\instGiessen} % 2416
  \author{R.~Giordano}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2103
  \author{A.~Giri}\affiliation{\instIITHyderabad} % 2106
  \author{A.~Glazov}\affiliation{\instDESY} % 2473
  \author{B.~Gobbo}\affiliation{\instTriesteINFN} % 2109
  \author{R.~Godang}\affiliation{\instSAlabama} % 2449
  \author{P.~Goldenzweig}\affiliation{\instKarlsruhe} % 2345
  \author{B.~Golob}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 3703
  \author{P.~Gomis}\affiliation{\instIFIC} % 2354
  \author{P.~Grace}\affiliation{\instAdelaide} % 9563
  \author{W.~Gradl}\affiliation{\instMainz} % 2570
  \author{E.~Graziani}\affiliation{\instRomaTreINFN} % 2342
  \author{D.~Greenwald}\affiliation{\instTUM} % 2686
  \author{Y.~Guan}\affiliation{\instCincinnati} % 2514
  \author{C.~Hadjivasiliou}\affiliation{\instPNNL} % 9503
  \author{S.~Halder}\affiliation{\instTata} % 4743
  \author{K.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2462
  \author{T.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2523
  \author{O.~Hartbrich}\affiliation{\instHawaii} % 2158
  \author{T.~Hauth}\affiliation{\instKarlsruhe} % 2553
  \author{K.~Hayasaka}\affiliation{\instNiigata} % 2330
  \author{H.~Hayashii}\affiliation{\instNaraWu} % 2455
  \author{C.~Hearty}\affiliation{\instUBC}\affiliation{\instIPP} % 2450
  \author{M.~Heck}\affiliation{\instKarlsruhe} % 2561
  \author{M.~T.~Hedges}\affiliation{\instHawaii} % 2265
  \author{I.~Heredia~de~la~Cruz}\affiliation{\instCinvestavIPN}\affiliation{\instConacyt} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva}\affiliation{\instMississippi} % 2466
  \author{A.~Hershenhorn}\affiliation{\instUBC} % 2552
  \author{T.~Higuchi}\affiliation{\instIPMU} % 2485
  \author{E.~C.~Hill}\affiliation{\instUBC} % 7823
  \author{H.~Hirata}\affiliation{\instNagoya} % 2070
  \author{M.~Hoek}\affiliation{\instMainz} % 2101
  \author{M.~Hohmann}\affiliation{\instMelbourne} % 2077
  \author{S.~Hollitt}\affiliation{\instAdelaide} % 2557
  \author{T.~Hotta}\affiliation{\instRCNP} % 2084
  \author{C.-L.~Hsu}\affiliation{\instSydney} % 2299
  \author{Y.~Hu}\affiliation{\instIHEPChina} % 2227
  \author{K.~Huang}\affiliation{\instNTUTaiwan} % 2389
  \author{T.~Iijima}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2446
  \author{K.~Inami}\affiliation{\instNagoya} % 2323
  \author{G.~Inguglia}\affiliation{\instHEPHYVienna} % 2500
  \author{J.~Irakkathil~Jabbar}\affiliation{\instKarlsruhe} % 7343
  \author{A.~Ishikawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2281
  \author{R.~Itoh}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2487
  \author{M.~Iwasaki}\affiliation{\instOsakaCity} % 2360
  \author{Y.~Iwasaki}\affiliation{\instKEK} % 2229
  \author{S.~Iwata}\affiliation{\instTokyoMetropolitan} % 4323
  \author{P.~Jackson}\affiliation{\instAdelaide} % 2255
  \author{W.~W.~Jacobs}\affiliation{\instIndiana} % 2322
  \author{I.~Jaegle}\affiliation{\instFlorida} % 2539
  \author{D.~E.~Jaffe}\affiliation{\instBNL} % 3663
  \author{E.-J.~Jang}\affiliation{\instGyeongsang} % 6744
  \author{M.~Jeandron}\affiliation{\instMississippi} % 2806
  \author{H.~B.~Jeon}\affiliation{\instKyungpook} % 2170
  \author{S.~Jia}\affiliation{\instFudan} % 2457
  \author{Y.~Jin}\affiliation{\instTriesteINFN} % 2105
  \author{C.~Joo}\affiliation{\instIPMU} % 3525
  \author{K.~K.~Joo}\affiliation{\instChonnam} % 4224
  \author{I.~Kadenko}\affiliation{\instKyiv} % 3843
  \author{J.~Kahn}\affiliation{\instKarlsruhe} % 2448
  \author{H.~Kakuno}\affiliation{\instTokyoMetropolitan} % 2391
  \author{A.~B.~Kaliyar}\affiliation{\instTata} % 7344
  \author{J.~Kandra}\affiliation{\instPrague} % 2541
  \author{K.~H.~Kang}\affiliation{\instKyungpook} % 2283
  \author{P.~Kapusta}\affiliation{\instKrakow} % 6663
  \author{R.~Karl}\affiliation{\instDESY} % 10923
  \author{G.~Karyan}\affiliation{\instYerevan} % 2550
  \author{Y.~Kato}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2549
  \author{H.~Kawai}\affiliation{\instChiba} % 4344
  \author{T.~Kawasaki}\affiliation{\instKitasato} % 4363
  \author{T.~Keck}\affiliation{\instKarlsruhe} % 2300
  \author{C.~Ketter}\affiliation{\instHawaii} % 2236
  \author{H.~Kichimi}\affiliation{\instKEK} % 2233
  \author{C.~Kiesling}\affiliation{\instMPP} % 2168
  \author{B.~H.~Kim}\affiliation{\instSeoul} % 9743
  \author{C.-H.~Kim}\affiliation{\instHanyang} % 2358
  \author{D.~Y.~Kim}\affiliation{\instSoongsil} % 2315
  \author{H.~J.~Kim}\affiliation{\instKyungpook} % 4863
  \author{J.~B.~Kim}\affiliation{\instKorea} % 2408
  \author{K.-H.~Kim}\affiliation{\instYonsei} % 2118
  \author{K.~Kim}\affiliation{\instKorea} % 2409
  \author{S.-H.~Kim}\affiliation{\instSeoul} % 2428
  \author{Y.-K.~Kim}\affiliation{\instYonsei} % 2379
  \author{Y.~Kim}\affiliation{\instKorea} % 2403
  \author{T.~D.~Kimmel}\affiliation{\instVPI} % 2241
  \author{H.~Kindo}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2195
  \author{K.~Kinoshita}\affiliation{\instCincinnati} % 2318
  \author{B.~Kirby}\affiliation{\instBNL} % 5263
  \author{C.~Kleinwort}\affiliation{\instDESY} % 2499
  \author{B.~Knysh}\affiliation{\instIJCLab} % 8883
  \author{P.~Kody\v{s}}\affiliation{\instPrague} % 2407
  \author{T.~Koga}\affiliation{\instKEK} % 6963
  \author{S.~Kohani}\affiliation{\instHawaii} % 9143
  \author{I.~Komarov}\affiliation{\instDESY} % 2210
  \author{T.~Konno}\affiliation{\instKitasato} % 2490
  \author{S.~Korpar}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % 2475
% \author{E.~Kou}\affiliation{\instIJCLab} % 3765
  \author{N.~Kovalchuk}\affiliation{\instDESY} % 6964
  \author{T.~M.~G.~Kraetzschmar}\affiliation{\instMPP} % 7543
  \author{P.~Kri\v{z}an}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2474
  \author{R.~Kroeger}\affiliation{\instMississippi} % 2242
  \author{J.~F.~Krohn}\affiliation{\instMelbourne} % 2502
  \author{P.~Krokovny}\affiliation{\instBINP}\affiliation{\instNSU} % 2575
  \author{H.~Kr\"uger}\affiliation{\instBonn} % 2290
  \author{W.~Kuehn}\affiliation{\instGiessen} % 2534
  \author{T.~Kuhr}\affiliation{\instLMU} % 2486
  \author{J.~Kumar}\affiliation{\instCMU} % 6464
  \author{M.~Kumar}\affiliation{\instMNITJaipur} % 2744
  \author{R.~Kumar}\affiliation{\instPanjabPAU} % 2189
  \author{K.~Kumara}\affiliation{\instWayneState} % 2257
  \author{T.~Kumita}\affiliation{\instTokyoMetropolitan} % 4083
  \author{T.~Kunigo}\affiliation{\instKEK} % 10104
  \author{M.~K\"{u}nzel}\affiliation{\instDESY}\affiliation{\instLMU} % 2139
  \author{S.~Kurz}\affiliation{\instDESY} % 9363
  \author{A.~Kuzmin}\affiliation{\instBINP}\affiliation{\instNSU} % 2520
  \author{P.~Kvasni\v{c}ka}\affiliation{\instPrague} % 2184
  \author{Y.-J.~Kwon}\affiliation{\instYonsei} % 2231
  \author{S.~Lacaprara}\affiliation{\instPadovaINFN} % 2447
  \author{Y.-T.~Lai}\affiliation{\instIPMU} % 2066
  \author{C.~La~Licata}\affiliation{\instIPMU} % 2348
  \author{K.~Lalwani}\affiliation{\instMNITJaipur} % 2142
  \author{L.~Lanceri}\affiliation{\instTriesteINFN} % 2540
  \author{J.~S.~Lange}\affiliation{\instGiessen} % 2277
  \author{K.~Lautenbach}\affiliation{\instGiessen} % 2102
  \author{P.~J.~Laycock}\affiliation{\instBNL} % 7683
  \author{F.~R.~Le~Diberder}\affiliation{\instIJCLab} % 3267
  \author{I.-S.~Lee}\affiliation{\instHanyang} % 2422
  \author{S.~C.~Lee}\affiliation{\instKyungpook} % 2544
  \author{P.~Leitl}\affiliation{\instMPP} % 2414
  \author{D.~Levit}\affiliation{\instTUM} % 2507
  \author{P.~M.~Lewis}\affiliation{\instBonn} % 2582
  \author{C.~Li}\affiliation{\instLNNU} % 2325
  \author{C.-H.~Li}\affiliation{\instNTUTaiwan} % 2884  
  \author{L.~K.~Li}\affiliation{\instCincinnati} % 3263
  \author{S.~X.~Li}\affiliation{\instBeihang} % 2377
  \author{Y.~M.~Li}\affiliation{\instIHEPChina} % 2203
  \author{Y.~B.~Li}\affiliation{\instPeking} % 2573
  \author{J.~Libby}\affiliation{\instIITMadras} % 2262
  \author{K.~Lieret}\affiliation{\instLMU} % 2268
  \author{L.~Li~Gioi}\affiliation{\instMPP} % 2495
  \author{J.~Lin}\affiliation{\instNTUTaiwan} % 2401
  \author{Z.~Liptak}\affiliation{\instHawaii} % 3565
  \author{Q.~Y.~Liu}\affiliation{\instDESY} % 7045
  \author{Z.~A.~Liu}\affiliation{\instIHEPChina} % 3283
  \author{D.~Liventsev}\affiliation{\instWayneState}\affiliation{\instKEK} % 2578
  \author{S.~Longo}\affiliation{\instDESY} % 2396
  \author{A.~Loos}\affiliation{\instSCarolina} % 2356
  \author{P.~Lu}\affiliation{\instNTUTaiwan} % 2148
  \author{M.~Lubej}\affiliation{\instLjubljanaJSI} % 2513
  \author{T.~Lueck}\affiliation{\instLMU} % 2406
  \author{F.~Luetticke}\affiliation{\instBonn} % 2533
  \author{T.~Luo}\affiliation{\instFudan} % 3268
  \author{C.~MacQueen}\affiliation{\instMelbourne} % 2585
  \author{Y.~Maeda}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2427
  \author{M.~Maggiora}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 5343
  \author{S.~Maity}\affiliation{\instIITBhubaneswar} % 2985
  \author{R.~Manfredi}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 10303
  \author{E.~Manoni}\affiliation{\instPerugiaINFN} % 2305
  \author{S.~Marcello}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 4223
  \author{C.~Marinas}\affiliation{\instIFIC} % 2133
  \author{A.~Martini}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 2336
  \author{M.~Masuda}\affiliation{\instEri}\affiliation{\instRCNP} % 2238
  \author{T.~Matsuda}\affiliation{\instUOM} % 5543
  \author{K.~Matsuoka}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2316
  \author{D.~Matvienko}\affiliation{\instBINP}\affiliation{\instLPI}\affiliation{\instNSU} % 2351
  \author{J.~McNeil}\affiliation{\instFlorida} % 2382
  \author{F.~Meggendorfer}\affiliation{\instMPP} % 7103
  \author{J.~C.~Mei}\affiliation{\instFudan} % 7404
  \author{F.~Meier}\affiliation{\instDuke} % 3103
  \author{M.~Merola}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2456
  \author{F.~Metzner}\affiliation{\instKarlsruhe} % 2296
  \author{M.~Milesi}\affiliation{\instMelbourne} % 5443
  \author{C.~Miller}\affiliation{\instVictoria} % 2273
  \author{K.~Miyabayashi}\affiliation{\instNaraWu} % 2327
  \author{H.~Miyake}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2452
  \author{H.~Miyata}\affiliation{\instNiigata} % 2071
  \author{R.~Mizuk}\affiliation{\instLPI}\affiliation{\instHSE} % 2483
  \author{K.~Azmi}\affiliation{\instMalaya} % 2506
  \author{G.~B.~Mohanty}\affiliation{\instTata} % 2278
  \author{H.~Moon}\affiliation{\instKorea} % 2304
  \author{T.~Moon}\affiliation{\instSeoul} % 2397
  \author{J.~A.~Mora~Grimaldo}\affiliation{\instUTokyo} % 4403
  \author{A.~Morda}\affiliation{\instPadovaINFN} % 2503
  \author{T.~Morii}\affiliation{\instIPMU} % 3543
  \author{H.-G.~Moser}\affiliation{\instMPP} % 2120
  \author{M.~Mrvar}\affiliation{\instHEPHYVienna} % 2527
  \author{F.~Mueller}\affiliation{\instMPP} % 2240
  \author{F.~J.~M\"{u}ller}\affiliation{\instDESY} % 2123
  \author{Th.~Muller}\affiliation{\instKarlsruhe} % 2165
  \author{G.~Muroyama}\affiliation{\instNagoya} % 2093
  \author{C.~Murphy}\affiliation{\instIPMU} % 12403
  \author{R.~Mussa}\affiliation{\instTorinoINFN} % 2372
  \author{K.~Nakagiri}\affiliation{\instKEK} % 10103
  \author{I.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 3463
  \author{K.~R.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2417
  \author{E.~Nakano}\affiliation{\instOsakaCity} % 2554
  \author{M.~Nakao}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2498
  \author{H.~Nakayama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2232
  \author{H.~Nakazawa}\affiliation{\instNTUTaiwan} % 2335
  \author{T.~Nanut}\affiliation{\instLjubljanaJSI} % 2565
  \author{Z.~Natkaniec}\affiliation{\instKrakow} % 3923
  \author{A.~Natochii}\affiliation{\instHawaii} % 12063
  \author{M.~Nayak}\affiliation{\instTelAviv} % 2371
  \author{G.~Nazaryan}\affiliation{\instYerevan} % 9523
  \author{D.~Neverov}\affiliation{\instNagoya} % 2075
  \author{C.~Niebuhr}\affiliation{\instDESY} % 2477
  \author{M.~Niiyama}\affiliation{\instKSU} % 2063
  \author{J.~Ninkovic}\affiliation{\instMPGHLL} % 2386
  \author{N.~K.~Nisar}\affiliation{\instBNL} % 2522
  \author{S.~Nishida}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2571
  \author{K.~Nishimura}\affiliation{\instHawaii} % 3063
  \author{M.~Nishimura}\affiliation{\instKEK} % 7743
  \author{M.~H.~A.~Nouxman}\affiliation{\instMalaya} % 2470
  \author{B.~Oberhof}\affiliation{\instFrascati} % 2393
  \author{K.~Ogawa}\affiliation{\instNiigata} % 2430
  \author{S.~Ogawa}\affiliation{\instToho} % 6263
  \author{S.~L.~Olsen}\affiliation{\instGyeongsang} % 4563
  \author{Y.~Onishchuk}\affiliation{\instKyiv} % 2157
  \author{H.~Ono}\affiliation{\instNiigata} % 2160
  \author{Y.~Onuki}\affiliation{\instUTokyo} % 2331
  \author{P.~Oskin}\affiliation{\instLPI} % 9623
  \author{E.~R.~Oxford}\affiliation{\instCMU} % 6943
  \author{H.~Ozaki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2984
  \author{P.~Pakhlov}\affiliation{\instLPI}\affiliation{\instMEPhI} % 2221
  \author{G.~Pakhlova}\affiliation{\instHSE}\affiliation{\instLPI} % 2188
  \author{A.~Paladino}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2435
  \author{T.~Pang}\affiliation{\instPittsburgh} % 2114
  \author{A.~Panta}\affiliation{\instMississippi} % 7943
  \author{E.~Paoloni}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2488
  \author{S.~Pardi}\affiliation{\instNapoliINFN} % 2532
  \author{C.~Park}\affiliation{\instYonsei} % 2307
  \author{H.~Park}\affiliation{\instKyungpook} % 2284
  \author{S.-H.~Park}\affiliation{\instYonsei} % 2509
  \author{B.~Paschen}\affiliation{\instBonn} % 2159
  \author{A.~Passeri}\affiliation{\instRomaTreINFN} % 2116
  \author{A.~Pathak}\affiliation{\instLouisville} % 8723
  \author{S.~Patra}\affiliation{\instIISER} % 3123
  \author{S.~Paul}\affiliation{\instTUM} % 2131
  \author{T.~K.~Pedlar}\affiliation{\instLuther} % 2421
  \author{I.~Peruzzi}\affiliation{\instFrascati} % 2253
  \author{R.~Peschke}\affiliation{\instHawaii} % 7123
  \author{R.~Pestotnik}\affiliation{\instLjubljanaJSI} % 2476
  \author{M.~Piccolo}\affiliation{\instFrascati} % 2147
  \author{L.~E.~Piilonen}\affiliation{\instVPI} % 2346
  \author{P.~L.~M.~Podesta-Lerma}\affiliation{\instUAS} % 2266
  \author{G.~Polat}\affiliation{\instCPPM} % 9783
  \author{V.~Popov}\affiliation{\instHSE} % 2096
  \author{C.~Praz}\affiliation{\instDESY} % 2726
  \author{E.~Prencipe}\affiliation{\instJuelich} % 2219
  \author{M.~T.~Prim}\affiliation{\instBonn} % 2501
  \author{M.~V.~Purohit}\affiliation{\instOkinawa} % 2196
  \author{N.~Rad}\affiliation{\instDESY} % 11683
  \author{P.~Rados}\affiliation{\instDESY} % 7383
  \author{S.~Raiz}\affiliation{\instTriesteINFN} % 4564
  \author{R.~Rasheed}\affiliation{\instIPHC} % 3643
  \author{M.~Reif}\affiliation{\instMPP} % 8043
  \author{S.~Reiter}\affiliation{\instGiessen} % 2248
  \author{M.~Remnev}\affiliation{\instBINP}\affiliation{\instNSU} % 2785
  \author{P.~K.~Resmi}\affiliation{\instIITMadras} % 2588
  \author{I.~Ripp-Baudot}\affiliation{\instIPHC} % 2469
  \author{M.~Ritter}\affiliation{\instLMU} % 2580
  \author{M.~Ritzert}\affiliation{\instHeidelberg} % 2526
  \author{G.~Rizzo}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2579
  \author{L.~B.~Rizzuto}\affiliation{\instLjubljanaJSI} % 3746
  \author{S.~H.~Robertson}\affiliation{\instMcGill}\affiliation{\instIPP} % 2471
  \author{D.~Rodr\'{i}guez~P\'{e}rez}\affiliation{\instUAS} % 2176
  \author{J.~M.~Roney}\affiliation{\instVictoria}\affiliation{\instIPP} % 2244
  \author{C.~Rosenfeld}\affiliation{\instSCarolina} % 2082
  \author{A.~Rostomyan}\affiliation{\instDESY} % 2481
  \author{N.~Rout}\affiliation{\instIITMadras} % 2965
  \author{M.~Rozanska}\affiliation{\instKrakow} % 2205
  \author{G.~Russo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2388
  \author{D.~Sahoo}\affiliation{\instTata} % 2110
  \author{Y.~Sakai}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2175
  \author{D.~A.~Sanders}\affiliation{\instMississippi} % 2458
  \author{S.~Sandilya}\affiliation{\instCincinnati} % 2286
  \author{A.~Sangal}\affiliation{\instCincinnati} % 2384
  \author{L.~Santelj}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2185
  \author{P.~Sartori}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 4523
  \author{J.~Sasaki}\affiliation{\instUTokyo} % 4383
  \author{Y.~Sato}\affiliation{\instTohoku} % 5243
  \author{V.~Savinov}\affiliation{\instPittsburgh} % 2292
  \author{B.~Scavino}\affiliation{\instMainz} % 2518
  \author{M.~Schram}\affiliation{\instPNNL} % 2306
  \author{H.~Schreeck}\affiliation{\instGoettingen} % 2434
  \author{J.~Schueler}\affiliation{\instHawaii} % 2824
  \author{C.~Schwanda}\affiliation{\instHEPHYVienna} % 2108
  \author{A.~J.~Schwartz}\affiliation{\instCincinnati} % 2162
  \author{B.~Schwenker}\affiliation{\instGoettingen} % 2405
  \author{R.~M.~Seddon}\affiliation{\instMcGill} % 2314
  \author{Y.~Seino}\affiliation{\instNiigata} % 2517
  \author{A.~Selce}\affiliation{\instRomaUNIV}\affiliation{\instRomaINFN} % 9043
  \author{K.~Senyo}\affiliation{\instYamagata} % 2987
  \author{I.~S.~Seong}\affiliation{\instHawaii} % 2572
  \author{J.~Serrano}\affiliation{\instCPPM} % 12124
  \author{M.~E.~Sevior}\affiliation{\instMelbourne} % 2328
  \author{C.~Sfienti}\affiliation{\instMainz} % 2214
  \author{V.~Shebalin}\affiliation{\instHawaii} % 2339
  \author{C.~P.~Shen}\affiliation{\instBeihang} % 2464
  \author{H.~Shibuya}\affiliation{\instToho} % 2234
  \author{J.-G.~Shiu}\affiliation{\instNTUTaiwan} % 2412
  \author{B.~Shwartz}\affiliation{\instBINP}\affiliation{\instNSU} % 2122
  \author{A.~Sibidanov}\affiliation{\instVictoria} % 2419
  \author{F.~Simon}\affiliation{\instMPP} % 2164
  \author{J.~B.~Singh}\affiliation{\instPanjab} % 2903
  \author{S.~Skambraks}\affiliation{\instMPP} % 2394
  \author{K.~Smith}\affiliation{\instMelbourne} % 2243
  \author{R.~J.~Sobie}\affiliation{\instVictoria}\affiliation{\instIPP} % 2472
  \author{A.~Soffer}\affiliation{\instTelAviv} % 2217
  \author{A.~Sokolov}\affiliation{\instIHEPRussia} % 2521
  \author{Y.~Soloviev}\affiliation{\instDESY} % 2479
  \author{E.~Solovieva}\affiliation{\instLPI} % 2398
  \author{S.~Spataro}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2117
  \author{B.~Spruck}\affiliation{\instMainz} % 2493
  \author{M.~Stari\v{c}}\affiliation{\instLjubljanaJSI} % 2326
  \author{S.~Stefkova}\affiliation{\instDESY} % 8783
  \author{Z.~S.~Stottler}\affiliation{\instVPI} % 2267
  \author{R.~Stroili}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 2465
  \author{J.~Strube}\affiliation{\instPNNL} % 2451
  \author{J.~Stypula}\affiliation{\instKrakow} % 2368
  \author{M.~Sumihama}\affiliation{\instGifu}\affiliation{\instRCNP} % 4243
  \author{K.~Sumisawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2583
  \author{T.~Sumiyoshi}\affiliation{\instTokyoMetropolitan} % 4184
  \author{D.~J.~Summers}\affiliation{\instMississippi} % 7405
  \author{W.~Sutcliffe}\affiliation{\instBonn} % 3784
  \author{K.~Suzuki}\affiliation{\instNagoya} % 2445
  \author{S.~Y.~Suzuki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2496
  \author{H.~Svidras}\affiliation{\instDESY} % 11783
  \author{M.~Tabata}\affiliation{\instChiba} % 2986
  \author{M.~Takahashi}\affiliation{\instDESY} % 2467
  \author{M.~Takizawa}\affiliation{\instRIKENMSL}\affiliation{\instJPARC}\affiliation{\instSPU} % 2437
  \author{U.~Tamponi}\affiliation{\instTorinoINFN} % 2366
  \author{S.~Tanaka}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2530
  \author{K.~Tanida}\affiliation{\instJAEA} % 3803
  \author{H.~Tanigawa}\affiliation{\instUTokyo} % 2237
  \author{N.~Taniguchi}\affiliation{\instKEK} % 2285
  \author{Y.~Tao}\affiliation{\instFlorida} % 2362
  \author{P.~Taras}\affiliation{\instMontreal} % 2202
  \author{F.~Tenchini}\affiliation{\instDESY} % 2546
  \author{D.~Tonelli}\affiliation{\instTriesteINFN} % 4564
  \author{E.~Torassa}\affiliation{\instPadovaINFN} % 2556
  \author{K.~Trabelsi}\affiliation{\instIJCLab} % 2369
  \author{T.~Tsuboyama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2361
  \author{N.~Tsuzuki}\affiliation{\instNagoya} % 2352
  \author{M.~Uchida}\affiliation{\instTitech} % 2370
  \author{I.~Ueda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2519
  \author{S.~Uehara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2586
  \author{T.~Ueno}\affiliation{\instTohoku} % 4364
  \author{T.~Uglov}\affiliation{\instLPI}\affiliation{\instHSE} % 2252
  \author{K.~Unger}\affiliation{\instKarlsruhe} % 9463
  \author{Y.~Unno}\affiliation{\instHanyang} % 2420
  \author{S.~Uno}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2149
  \author{P.~Urquijo}\affiliation{\instMelbourne} % 2302
  \author{Y.~Ushiroda}\affiliation{\instKEK}\affiliation{\instSOKENDAI}\affiliation{\instUTokyo} % 2317
  \author{Y.~Usov}\affiliation{\instBINP}\affiliation{\instNSU} % 5003
  \author{S.~E.~Vahsen}\affiliation{\instHawaii} % 2251
  \author{R.~van~Tonder}\affiliation{\instBonn} % 2706
  \author{G.~S.~Varner}\affiliation{\instHawaii} % 2119
  \author{K.~E.~Varvell}\affiliation{\instSydney} % 2545
  \author{A.~Vinokurova}\affiliation{\instBINP}\affiliation{\instNSU} % 2289
  \author{L.~Vitale}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 2415
  \author{V.~Vorobyev}\affiliation{\instBINP}\affiliation{\instLPI}\affiliation{\instNSU} % 2298
  \author{A.~Vossen}\affiliation{\instDuke} % 2249
  \author{B.~Wach}\affiliation{\instMPP} % 2120  
  \author{E.~Waheed}\affiliation{\instKEK} % 2226
  \author{H.~M.~Wakeling}\affiliation{\instMcGill} % 3664
  \author{K.~Wan}\affiliation{\instUTokyo} % 2591
  \author{W.~Wan~Abdullah}\affiliation{\instMalaya} % 2280
  \author{B.~Wang}\affiliation{\instMPP} % 2569
  \author{C.~H.~Wang}\affiliation{\instNUUTaiwan} % 2224
  \author{M.-Z.~Wang}\affiliation{\instNTUTaiwan} % 2074
  \author{X.~L.~Wang}\affiliation{\instFudan} % 2076
  \author{A.~Warburton}\affiliation{\instMcGill} % 2347
  \author{M.~Watanabe}\affiliation{\instNiigata} % 2309
  \author{S.~Watanuki}\affiliation{\instIJCLab} % 6843
  \author{I.~Watson}\affiliation{\instUTokyo} % 2337
  \author{J.~Webb}\affiliation{\instMelbourne} % 2423
  \author{S.~Wehle}\affiliation{\instDESY} % 2489
  \author{M.~Welsch}\affiliation{\instBonn} % 7023
  \author{C.~Wessel}\affiliation{\instBonn} % 2100
  \author{J.~Wiechczynski}\affiliation{\instPisaINFN} % 2604
  \author{P.~Wieduwilt}\affiliation{\instGoettingen} % 2343
  \author{H.~Windel}\affiliation{\instMPP} % 2081
  \author{E.~Won}\affiliation{\instKorea} % 2410
  \author{L.~J.~Wu}\affiliation{\instIHEPChina} % 2704
  \author{X.~P.~Xu}\affiliation{\instSoochow} % 4923
  \author{B.~Yabsley}\affiliation{\instSydney} % 3645
  \author{S.~Yamada}\affiliation{\instKEK} % 2492
  \author{W.~Yan}\affiliation{\instUSTC} % 2094
  \author{S.~B.~Yang}\affiliation{\instKorea} % 2374
  \author{H.~Ye}\affiliation{\instDESY} % 2537
  \author{J.~Yelton}\affiliation{\instFlorida} % 2067
  \author{I.~Yeo}\affiliation{\instKISTI} % 2204
  \author{J.~H.~Yin}\affiliation{\instKorea} % 2365
  \author{M.~Yonenaga}\affiliation{\instTokyoMetropolitan} % 2411
  \author{Y.~M.~Yook}\affiliation{\instIHEPChina} % 2453
  \author{T.~Yoshinobu}\affiliation{\instNiigata} % 2429
  \author{C.~Z.~Yuan}\affiliation{\instIHEPChina} % 2088
  \author{G.~Yuan}\affiliation{\instUSTC} % 7243
  \author{W.~Yuan}\affiliation{\instPadovaINFN} % 2504
  \author{Y.~Yusa}\affiliation{\instNiigata} % 2357
  \author{L.~Zani}\affiliation{\instCPPM} % 2529
  \author{J.~Z.~Zhang}\affiliation{\instIHEPChina} % 2349
  \author{Y.~Zhang}\affiliation{\instUSTC} % 2607
  \author{Z.~Zhang}\affiliation{\instUSTC} % 5363
  \author{V.~Zhilich}\affiliation{\instBINP}\affiliation{\instNSU} % 4703
  \author{Q.~D.~Zhou}\affiliation{\instNagoya}\affiliation{\instNagoyaIAR} % 7323
  \author{X.~Y.~Zhou}\affiliation{\instBeihang} % 2380
  \author{V.~I.~Zhukova}\affiliation{\instLPI} % 2387
  \author{V.~Zhulanov}\affiliation{\instBINP}\affiliation{\instNSU} % 4983
  \author{A.~Zupanc}\affiliation{\instLjubljanaJSI} % 2543
\collaboration{Belle II Collaboration}

==> belle2sym.tex <==
%%%%%   Standard symbols for use in Belle II notes and papers. 
%%%%%
%%%%%	C. Hearty	21-Oct-2014		Based on babarsym.tex; authored by D. Hitlin, D. MacFarlane, P. Dauncey, and R. Waldi
%%%%%


\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% THE NAME OF THE COLLABORATION %%%%
\def\belletwo {Belle~II}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\SixS  {\Y6S}

\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second 
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    


\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}

\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}






==> contents/Author.tex <==
%\input ./authors-conf2020.tex
%%% Paper:    (2020  conference papers)
%%% Journal:  (2020 conferences)
%%% ====================================================================
%%% Use \input{authors-conf2020} to insert this material into your latex file.
\newcommand{\instSinica}{Academia Sinica, Taipei 11529, Taiwan}
\newcommand{\instCPPM}{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\newcommand{\instBeihang}{Beihang University, Beijing 100191, China}
\newcommand{\instBUAP}{Benemerita Universidad Autonoma de Puebla, Puebla 72570, Mexico}
\newcommand{\instBNL}{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\newcommand{\instBINP}{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
\newcommand{\instCMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\newcommand{\instCinvestavIPN}{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\newcommand{\instPrague}{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\newcommand{\instChiangMai}{Chiang Mai University, Chiang Mai 50202, Thailand}
\newcommand{\instChiba}{Chiba University, Chiba 263-8522, Japan}
\newcommand{\instChonnam}{Chonnam National University, Gwangju 61186, South Korea}
\newcommand{\instConacyt}{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\newcommand{\instDESY}{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\newcommand{\instDuke}{Duke University, Durham, North Carolina 27708, U.S.A.}
\newcommand{\instITAR}{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
\newcommand{\instENEA}{ENEA Casaccia, I-00123 Roma, Italy}
\newcommand{\instEri}{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\newcommand{\instJuelich}{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich, Germany}
\newcommand{\instFuJen}{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\newcommand{\instFudan}{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\newcommand{\instGoettingen}{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
\newcommand{\instGifu}{Gifu University, Gifu 501-1193, Japan}
\newcommand{\instSOKENDAI}{The Graduate University for Advanced Studies (SOKENDAI), Hayama 240-0193, Japan}
\newcommand{\instGyeongsang}{Gyeongsang National University, Jinju 52828, South Korea}
\newcommand{\instHanyang}{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
\newcommand{\instKEK}{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instJPARC}{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instHSE}{Higher School of Economics (HSE), Moscow 101000, Russian Federation}
\newcommand{\instIISER}{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\newcommand{\instIITBhubaneswar}{Indian Institute of Technology Bhubaneswar, Satya Nagar 751007, India}
\newcommand{\instIITGuwahati}{Indian Institute of Technology Guwahati, Assam 781039, India}
\newcommand{\instIITHyderabad}{Indian Institute of Technology Hyderabad, Telangana 502285, India}
\newcommand{\instIITMadras}{Indian Institute of Technology Madras, Chennai 600036, India}
\newcommand{\instIndiana}{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\newcommand{\instIHEPRussia}{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\newcommand{\instHEPHYVienna}{Institute of High Energy Physics, Vienna 1050, Austria}
\newcommand{\instIHEPChina}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\newcommand{\instChennai}{Institute of Mathematical Sciences, Chennai 600113, India}
\newcommand{\instIPP}{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\newcommand{\instIOP}{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\newcommand{\instIFIC}{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\newcommand{\instFrascati}{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\newcommand{\instNapoliINFN}{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\newcommand{\instPadovaINFN}{INFN Sezione di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaINFN}{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaINFN}{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaINFN}{INFN Sezione di Roma, I-00185 Roma, Italy}
\newcommand{\instRomaTreINFN}{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoINFN}{INFN Sezione di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteINFN}{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\newcommand{\instJAEA}{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
\newcommand{\instMainz}{Johannes Gutenberg-Universit\"{a}t Mainz, Institut f\"{u}r Kernphysik, D-55099 Mainz, Germany}
\newcommand{\instGiessen}{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\newcommand{\instKarlsruhe}{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
\newcommand{\instKennesaw}{Kennesaw State University, Kennesaw, Georgia 30144, U.S.A.}
\newcommand{\instKitasato}{Kitasato University, Sagamihara 252-0373, Japan}
\newcommand{\instKISTI}{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\newcommand{\instKorea}{Korea University, Seoul 02841, South Korea}
\newcommand{\instKSU}{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\newcommand{\instKyotoU}{Kyoto University, Kyoto 606-8501, Japan}
\newcommand{\instKyungpook}{Kyungpook National University, Daegu 41566, South Korea}
\newcommand{\instLPI}{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991, Russian Federation}
\newcommand{\instLNNU}{Liaoning Normal University, Dalian 116029, China}
\newcommand{\instLMU}{Ludwig Maximilians University, 80539 Munich, Germany}
\newcommand{\instISUni}{Iowa State University,  Ames, Iowa 50011, U.S.A.}
\newcommand{\instLuther}{Luther College, Decorah, Iowa 52101, U.S.A.}
\newcommand{\instMNITJaipur}{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\newcommand{\instMPP}{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
\newcommand{\instMPGHLL}{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
\newcommand{\instMcGill}{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
\newcommand{\instMETU}{Middle East Technical University, 06531 Ankara, Turkey}
\newcommand{\instMEPhI}{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\newcommand{\instNagoya}{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaKMI}{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaIAR}{Institute for Advanced Research, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNaraWu}{Nara Women's University, Nara 630-8506, Japan}
\newcommand{\instUNAM}{National Autonomous University of Mexico, Mexico City, Mexico}
\newcommand{\instNTUTaiwan}{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
\newcommand{\instNUUTaiwan}{National United University, Miao Li 36003, Taiwan}
\newcommand{\instKrakow}{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\newcommand{\instNiigata}{Niigata University, Niigata 950-2181, Japan}
\newcommand{\instNSU}{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\newcommand{\instOkinawa}{Okinawa Institute of Science and Technology, Okinawa 904-0495, Japan}
\newcommand{\instOsakaCity}{Osaka City University, Osaka 558-8585, Japan}
\newcommand{\instRCNP}{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\newcommand{\instPNNL}{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\newcommand{\instPanjab}{Panjab University, Chandigarh 160014, India}
\newcommand{\instPeking}{Peking University, Beijing 100871, China}
\newcommand{\instPanjabPAU}{Punjab Agricultural University, Ludhiana 141004, India}
\newcommand{\instRIKENMSL}{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
\newcommand{\instRIKEN}{Theoretical Research Division, Nishina Center, RIKEN, Saitama 351-0198, Japan}
\newcommand{\instXavier}{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\newcommand{\instSeoul}{Seoul National University, Seoul 08826, South Korea}
\newcommand{\instShandong}{Shandong University, Jinan 250100, China}
\newcommand{\instSPU}{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\newcommand{\instSoochow}{Soochow University, Suzhou 215006, China}
\newcommand{\instSoongsil}{Soongsil University, Seoul 06978, South Korea}
\newcommand{\instLjubljanaJSI}{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\newcommand{\instKyiv}{Taras Shevchenko National Univ. of Kiev, Kiev, Ukraine}
\newcommand{\instTata}{Tata Institute of Fundamental Research, Mumbai 400005, India}
\newcommand{\instTUM}{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\newcommand{\instECUTUM}{Excellence Cluster Universe, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\newcommand{\instTelAviv}{Tel Aviv University, School of Physics and Astronomy, Tel Aviv, 69978, Israel}
\newcommand{\instToho}{Toho University, Funabashi 274-8510, Japan}
\newcommand{\instTohoku}{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
\newcommand{\instTitech}{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
\newcommand{\instTokyoMetropolitan}{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\newcommand{\instUAS}{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
\newcommand{\instNapoliUNIV}{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\newcommand{\instNapoliUNIVA}{Dipartimento di Agraria, Universit\`{a} di Napoli Federico II, I-80055 Portici (NA), Italy}
\newcommand{\instPadovaUNIV}{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaUNIV}{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaUNIV}{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaUNIV}{Universit\`{a} di Roma ``La Sapienza,'' I-00185 Roma, Italy}
\newcommand{\instRomaTreUNIV}{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoUNIV}{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteUNIV}{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
\newcommand{\instMontreal}{Universit\'{e} de Montr\'{e}al, Physique des Particules, Montr\'{e}al, Qu\'{e}bec, H3C 3J7, Canada}
\newcommand{\instIJCLab}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\newcommand{\instIPHC}{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\newcommand{\instAdelaide}{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
\newcommand{\instBonn}{University of Bonn, 53115 Bonn, Germany}
\newcommand{\instUBC}{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\newcommand{\instCincinnati}{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\newcommand{\instFlorida}{University of Florida, Gainesville, Florida 32611, U.S.A.}
\newcommand{\instHamburg}{University of Hamburg, 20148 Hamburg, Germany}
\newcommand{\instHawaii}{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\newcommand{\instHeidelberg}{University of Heidelberg, 68131 Mannheim, Germany}
\newcommand{\instLjubljanaUniLJ}{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\newcommand{\instLouisville}{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
\newcommand{\instMalaya}{National Centre for Particle Physics, University Malaya, 50603 Kuala Lumpur, Malaysia}
\newcommand{\instLjubljanaUM}{University of Maribor, 2000 Maribor, Slovenia}
\newcommand{\instMelbourne}{School of Physics, University of Melbourne, Victoria 3010, Australia}
\newcommand{\instMississippi}{University of Mississippi, University, Mississippi 38677, U.S.A.}
\newcommand{\instUOM}{University of Miyazaki, Miyazaki 889-2192, Japan}
\newcommand{\instNovaGorica}{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\newcommand{\instPittsburgh}{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\newcommand{\instUSTC}{University of Science and Technology of China, Hefei 230026, China}
\newcommand{\instSAlabama}{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
\newcommand{\instSCarolina}{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\newcommand{\instSydney}{School of Physics, University of Sydney, New South Wales 2006, Australia}
\newcommand{\instTabuk}{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\newcommand{\instUTokyo}{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\newcommand{\instIPMU}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\newcommand{\instVictoria}{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\newcommand{\instVPI}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\newcommand{\instWayneState}{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\newcommand{\instYamagata}{Yamagata University, Yamagata 990-8560, Japan}
\newcommand{\instYerevan}{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
\newcommand{\instYonsei}{Yonsei University, Seoul 03722, South Korea}
%%%\affiliation{\instSinica}
\affiliation{\instCPPM}
\affiliation{\instBeihang}
%%%\affiliation{\instBUAP}
\affiliation{\instBNL}
\affiliation{\instBINP}
\affiliation{\instCMU}
\affiliation{\instCinvestavIPN}
\affiliation{\instPrague}
\affiliation{\instChiangMai}
\affiliation{\instChiba}
\affiliation{\instChonnam}
\affiliation{\instConacyt}
\affiliation{\instDESY}
\affiliation{\instDuke}
\affiliation{\instITAR}
%%%\affiliation{\instENEA}
\affiliation{\instEri}
\affiliation{\instJuelich}
\affiliation{\instFuJen}
\affiliation{\instFudan}
\affiliation{\instGoettingen}
\affiliation{\instGifu}
\affiliation{\instSOKENDAI}
\affiliation{\instGyeongsang}
\affiliation{\instHanyang}
\affiliation{\instKEK}
\affiliation{\instJPARC}
\affiliation{\instHSE}
\affiliation{\instIISER}
\affiliation{\instIITBhubaneswar}
\affiliation{\instIITGuwahati}
\affiliation{\instIITHyderabad}
\affiliation{\instIITMadras}
\affiliation{\instIndiana}
\affiliation{\instIHEPRussia}
\affiliation{\instHEPHYVienna}
\affiliation{\instIHEPChina}
%%%\affiliation{\instChennai}
\affiliation{\instIPP}
\affiliation{\instIOP}
\affiliation{\instIFIC}
\affiliation{\instFrascati}
\affiliation{\instNapoliINFN}
\affiliation{\instPadovaINFN}
\affiliation{\instPerugiaINFN}
\affiliation{\instPisaINFN}
\affiliation{\instRomaINFN}
\affiliation{\instRomaTreINFN}
\affiliation{\instTorinoINFN}
\affiliation{\instTriesteINFN}
\affiliation{\instISUni}
\affiliation{\instJAEA}
\affiliation{\instMainz}
\affiliation{\instGiessen}
\affiliation{\instKarlsruhe}
%%%\affiliation{\instKennesaw}
\affiliation{\instKitasato}
\affiliation{\instKISTI}
\affiliation{\instKorea}
\affiliation{\instKSU}
%%%\affiliation{\instKyotoU}
\affiliation{\instKyungpook}
\affiliation{\instLPI}
\affiliation{\instLNNU}
\affiliation{\instLMU}
\affiliation{\instLuther}
\affiliation{\instMNITJaipur}
\affiliation{\instMPP}
\affiliation{\instMPGHLL}
\affiliation{\instMcGill}
%%%\affiliation{\instMETU}
\affiliation{\instMEPhI}
\affiliation{\instNagoya}
\affiliation{\instNagoyaKMI}
\affiliation{\instNagoyaIAR}
\affiliation{\instNaraWu}
%%%\affiliation{\instUNAM}
\affiliation{\instNTUTaiwan}
\affiliation{\instNUUTaiwan}
\affiliation{\instKrakow}
\affiliation{\instNiigata}
\affiliation{\instNSU}
\affiliation{\instOkinawa}
\affiliation{\instOsakaCity}
\affiliation{\instRCNP}
\affiliation{\instPNNL}
\affiliation{\instPanjab}
\affiliation{\instPeking}
\affiliation{\instPanjabPAU}
\affiliation{\instRIKENMSL}
%%%\affiliation{\instRIKEN}
%%%\affiliation{\instXavier}
\affiliation{\instSeoul}
%%%\affiliation{\instShandong}
\affiliation{\instSPU}
\affiliation{\instSoochow}
\affiliation{\instSoongsil}
\affiliation{\instLjubljanaJSI}
\affiliation{\instKyiv}
\affiliation{\instTata}
\affiliation{\instTUM}
%%%\affiliation{\instECUTUM}
\affiliation{\instTelAviv}
\affiliation{\instToho}
\affiliation{\instTohoku}
\affiliation{\instTitech}
\affiliation{\instTokyoMetropolitan}
\affiliation{\instUAS}
\affiliation{\instNapoliUNIV}
\affiliation{\instPadovaUNIV}
\affiliation{\instPerugiaUNIV}
\affiliation{\instPisaUNIV}
\affiliation{\instRomaUNIV}
\affiliation{\instRomaTreUNIV}
\affiliation{\instTorinoUNIV}
\affiliation{\instTriesteUNIV}
\affiliation{\instMontreal}
\affiliation{\instIJCLab}
\affiliation{\instIPHC}
\affiliation{\instAdelaide}
\affiliation{\instBonn}
\affiliation{\instUBC}
\affiliation{\instCincinnati}
\affiliation{\instFlorida}
%%%\affiliation{\instHamburg}
\affiliation{\instHawaii}
\affiliation{\instHeidelberg}
\affiliation{\instLjubljanaUniLJ}
\affiliation{\instLouisville}
\affiliation{\instMalaya}
\affiliation{\instLjubljanaUM}
\affiliation{\instMelbourne}
\affiliation{\instMississippi}
\affiliation{\instUOM}
%%%\affiliation{\instNovaGorica}
\affiliation{\instPittsburgh}
\affiliation{\instUSTC}
\affiliation{\instSAlabama}
\affiliation{\instSCarolina}
\affiliation{\instSydney}
%%%\affiliation{\instTabuk}
\affiliation{\instUTokyo}
\affiliation{\instIPMU}
\affiliation{\instVictoria}
\affiliation{\instVPI}
\affiliation{\instWayneState}
\affiliation{\instYamagata}
\affiliation{\instYerevan}
\affiliation{\instYonsei}
  \author{F.~Abudin{\'e}n}\affiliation{\instTriesteINFN} % 2250
  \author{I.~Adachi}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2590
  \author{R.~Adak}\affiliation{\instFudan} % 6743
  \author{K.~Adamczyk}\affiliation{\instKrakow} % 2239
  \author{P.~Ahlburg}\affiliation{\instBonn} % 2367
  \author{J.~K.~Ahn}\affiliation{\instKorea} % 7423
  \author{H.~Aihara}\affiliation{\instUTokyo} % 2223
  \author{N.~Akopov}\affiliation{\instYerevan} % 9443
  \author{A.~Aloisio}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2194
  \author{F.~Ameli}\affiliation{\instRomaINFN} % 4683
  \author{L.~Andricek}\affiliation{\instMPGHLL} % 2098
  \author{N.~Anh~Ky}\affiliation{\instIOP}\affiliation{\instITAR} % 2218
  \author{D.~M.~Asner}\affiliation{\instBNL} % 4684
  \author{H.~Atmacan}\affiliation{\instCincinnati} % 2538
  \author{V.~Aulchenko}\affiliation{\instBINP}\affiliation{\instNSU} % 8183
  \author{T.~Aushev}\affiliation{\instHSE} % 3747
  \author{V.~Aushev}\affiliation{\instKyiv} % 2155
  \author{T.~Aziz}\affiliation{\instTata} % 3523
  \author{V.~Babu}\affiliation{\instDESY} % 5623
  \author{S.~Bacher}\affiliation{\instKrakow} % 2258
  \author{S.~Baehr}\affiliation{\instKarlsruhe} % 2515
  \author{S.~Bahinipati}\affiliation{\instIITBhubaneswar} % 2332
  \author{A.~M.~Bakich}\affiliation{\instSydney} % 2115
  \author{P.~Bambade}\affiliation{\instIJCLab} % 3003
  \author{Sw.~Banerjee}\affiliation{\instLouisville} % 8603
  \author{S.~Bansal}\affiliation{\instPanjab} % 5163
  \author{M.~Barrett}\affiliation{\instKEK} % 2180
  \author{G.~Batignani}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 6643
  \author{J.~Baudot}\affiliation{\instIPHC} % 2562
  \author{A.~Beaulieu}\affiliation{\instVictoria} % 2444
  \author{J.~Becker}\affiliation{\instKarlsruhe} % 5403
  \author{P.~K.~Behera}\affiliation{\instIITMadras} % 4204
  \author{M.~Bender}\affiliation{\instLMU} % 2440
  \author{J.~V.~Bennett}\affiliation{\instMississippi} % 2454
  \author{E.~Bernieri}\affiliation{\instRomaTreINFN} % 4483
  \author{F.~U.~Bernlochner}\affiliation{\instBonn} % 2282
  \author{M.~Bertemes}\affiliation{\instHEPHYVienna} % 2595
  \author{M.~Bessner}\affiliation{\instHawaii} % 3783
  \author{S.~Bettarini}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2350
  \author{V.~Bhardwaj}\affiliation{\instIISER} % 2228
  \author{B.~Bhuyan}\affiliation{\instIITGuwahati} % 2097
  \author{F.~Bianchi}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2564
  \author{T.~Bilka}\affiliation{\instPrague} % 2484
  \author{S.~Bilokin}\affiliation{\instLMU} % 3623
  \author{D.~Biswas}\affiliation{\instLouisville} % 8703
  \author{A.~Bobrov}\affiliation{\instBINP}\affiliation{\instNSU} % 2294
  \author{A.~Bondar}\affiliation{\instBINP}\affiliation{\instNSU} % 4643
  \author{G.~Bonvicini}\affiliation{\instWayneState} % 2095
  \author{A.~Bozek}\affiliation{\instKrakow} % 2303
  \author{M.~Bra\v{c}ko}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % 2425
  \author{P.~Branchini}\affiliation{\instRomaTreINFN} % 2577
  \author{N.~Braun}\affiliation{\instKarlsruhe} % 2436
  \author{R.~A.~Briere}\affiliation{\instCMU} % 2584
  \author{T.~E.~Browder}\affiliation{\instHawaii} % 2560
  \author{D.~N.~Brown}\affiliation{\instLouisville} % 8743
  \author{A.~Budano}\affiliation{\instRomaTreINFN} % 2171
  \author{L.~Burmistrov}\affiliation{\instIJCLab} % 2111
  \author{S.~Bussino}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 5384
  \author{M.~Campajola}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 5223
  \author{L.~Cao}\affiliation{\instBonn} % 2099
  \author{G.~Caria}\affiliation{\instMelbourne} % 2438
  \author{G.~Casarosa}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2491
  \author{C.~Cecchi}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 2433
  \author{D.~\v{C}ervenkov}\affiliation{\instPrague} % 2078
  \author{M.-C.~Chang}\affiliation{\instFuJen} % 2827
  \author{P.~Chang}\affiliation{\instNTUTaiwan} % 2542
  \author{R.~Cheaib}\affiliation{\instUBC} % 2208
  \author{V.~Chekelian}\affiliation{\instMPP} % 2167
  \author{C.~Chen}\affiliation{\instISUni}
  \author{Y.-C.~Chen}\affiliation{\instNTUTaiwan} 
  \author{Y.~Q.~Chen}\affiliation{\instUSTC} % 2576
  \author{Y.-T.~Chen}\affiliation{\instNTUTaiwan} % 2884
  \author{B.~G.~Cheon}\affiliation{\instHanyang} % 2173
  \author{K.~Chilikin}\affiliation{\instLPI} % 2308
  \author{K.~Chirapatpimol}\affiliation{\instChiangMai} % 10803
  \author{H.-E.~Cho}\affiliation{\instHanyang} % 2182
  \author{K.~Cho}\affiliation{\instKISTI} % 2516
  \author{S.-J.~Cho}\affiliation{\instYonsei} % 2723
  \author{S.-K.~Choi}\affiliation{\instGyeongsang} % 2364
  \author{S.~Choudhury}\affiliation{\instIITHyderabad} % 2206
  \author{D.~Cinabro}\affiliation{\instWayneState} % 2092
  \author{L.~Corona}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 3944
  \author{L.~M.~Cremaldi}\affiliation{\instMississippi} % 2276
  \author{D.~Cuesta}\affiliation{\instIPHC} % 2668
  \author{S.~Cunliffe}\affiliation{\instDESY} % 2272
  \author{T.~Czank}\affiliation{\instIPMU} % 2254
  \author{N.~Dash}\affiliation{\instIITMadras} % 2601
  \author{F.~Dattola}\affiliation{\instDESY} % 3745
  \author{E.~De~La~Cruz-Burelo}\affiliation{\instCinvestavIPN} % 2359
  \author{G.~De~Nardo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2459
  \author{M.~De~Nuccio}\affiliation{\instDESY} % 2610
  \author{G.~De~Pietro}\affiliation{\instRomaTreINFN} % 2528
  \author{R.~de~Sangro}\affiliation{\instFrascati} % 2524
  \author{B.~Deschamps}\affiliation{\instBonn} % 2671
  \author{M.~Destefanis}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2594
  \author{S.~Dey}\affiliation{\instTelAviv} % 5023
  \author{A.~De~Yta-Hernandez}\affiliation{\instCinvestavIPN} % 2104
  \author{A.~Di~Canto}\affiliation{\instBNL} % 10963
  \author{F.~Di~Capua}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2065
  \author{S.~Di~Carlo}\affiliation{\instIJCLab} % 2079
  \author{J.~Dingfelder}\affiliation{\instBonn} % 2151
  \author{Z.~Dole\v{z}al}\affiliation{\instPrague} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez}\affiliation{\instUAS} % 2191
  \author{T.~V.~Dong}\affiliation{\instFudan} % 2215
  \author{K.~Dort}\affiliation{\instGiessen} % 5583
  \author{D.~Dossett}\affiliation{\instMelbourne} % 2574
  \author{S.~Dubey}\affiliation{\instHawaii} % 11063
  \author{S.~Duell}\affiliation{\instBonn} % 2344
  \author{G.~Dujany}\affiliation{\instIPHC} % 9703
  \author{S.~Eidelman}\affiliation{\instBINP}\affiliation{\instLPI}\affiliation{\instNSU} % 4984
  \author{M.~Eliachevitch}\affiliation{\instBonn} % 2725
  \author{D.~Epifanov}\affiliation{\instBINP}\affiliation{\instNSU} % 2551
  \author{J.~E.~Fast}\affiliation{\instPNNL} % 2264
  \author{T.~Ferber}\affiliation{\instDESY} % 2482
  \author{D.~Ferlewicz}\affiliation{\instMelbourne} % 2073
  \author{G.~Finocchiaro}\affiliation{\instFrascati} % 2400
  \author{S.~Fiore}\affiliation{\instRomaINFN} % 4225
  \author{P.~Fischer}\affiliation{\instHeidelberg} % 2141
  \author{A.~Fodor}\affiliation{\instMcGill} % 2312
  \author{F.~Forti}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2432
  \author{A.~Frey}\affiliation{\instGoettingen} % 2150
  \author{M.~Friedl}\affiliation{\instHEPHYVienna} % 2442
  \author{B.~G.~Fulsom}\affiliation{\instPNNL} % 2563
  \author{M.~Gabriel}\affiliation{\instMPP} % 2443
  \author{N.~Gabyshev}\affiliation{\instBINP}\affiliation{\instNSU} % 2510
  \author{E.~Ganiev}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 4623
  \author{M.~Garcia-Hernandez}\affiliation{\instCinvestavIPN} % 4823
  \author{R.~Garg}\affiliation{\instPanjab} % 2213
  \author{A.~Garmash}\affiliation{\instBINP}\affiliation{\instNSU} % 2161
  \author{V.~Gaur}\affiliation{\instVPI} % 2413
  \author{A.~Gaz}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2181
  \author{U.~Gebauer}\affiliation{\instGoettingen} % 2174
  \author{M.~Gelb}\affiliation{\instKarlsruhe} % 2340
  \author{A.~Gellrich}\affiliation{\instDESY} % 2480
  \author{J.~Gemmler}\affiliation{\instKarlsruhe} % 2321
  \author{T.~Ge{\ss}ler}\affiliation{\instGiessen} % 2121
  \author{D.~Getzkow}\affiliation{\instGiessen} % 2416
  \author{R.~Giordano}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2103
  \author{A.~Giri}\affiliation{\instIITHyderabad} % 2106
  \author{A.~Glazov}\affiliation{\instDESY} % 2473
  \author{B.~Gobbo}\affiliation{\instTriesteINFN} % 2109
  \author{R.~Godang}\affiliation{\instSAlabama} % 2449
  \author{P.~Goldenzweig}\affiliation{\instKarlsruhe} % 2345
  \author{B.~Golob}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 3703
  \author{P.~Gomis}\affiliation{\instIFIC} % 2354
  \author{P.~Grace}\affiliation{\instAdelaide} % 9563
  \author{W.~Gradl}\affiliation{\instMainz} % 2570
  \author{E.~Graziani}\affiliation{\instRomaTreINFN} % 2342
  \author{D.~Greenwald}\affiliation{\instTUM} % 2686
  \author{Y.~Guan}\affiliation{\instCincinnati} % 2514
  \author{C.~Hadjivasiliou}\affiliation{\instPNNL} % 9503
  \author{S.~Halder}\affiliation{\instTata} % 4743
  \author{K.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2462
  \author{T.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2523
  \author{O.~Hartbrich}\affiliation{\instHawaii} % 2158
  \author{T.~Hauth}\affiliation{\instKarlsruhe} % 2553
  \author{K.~Hayasaka}\affiliation{\instNiigata} % 2330
  \author{H.~Hayashii}\affiliation{\instNaraWu} % 2455
  \author{C.~Hearty}\affiliation{\instUBC}\affiliation{\instIPP} % 2450
  \author{M.~Heck}\affiliation{\instKarlsruhe} % 2561
  \author{M.~T.~Hedges}\affiliation{\instHawaii} % 2265
  \author{I.~Heredia~de~la~Cruz}\affiliation{\instCinvestavIPN}\affiliation{\instConacyt} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva}\affiliation{\instMississippi} % 2466
  \author{A.~Hershenhorn}\affiliation{\instUBC} % 2552
  \author{T.~Higuchi}\affiliation{\instIPMU} % 2485
  \author{E.~C.~Hill}\affiliation{\instUBC} % 7823
  \author{H.~Hirata}\affiliation{\instNagoya} % 2070
  \author{M.~Hoek}\affiliation{\instMainz} % 2101
  \author{M.~Hohmann}\affiliation{\instMelbourne} % 2077
  \author{S.~Hollitt}\affiliation{\instAdelaide} % 2557
  \author{T.~Hotta}\affiliation{\instRCNP} % 2084
  \author{C.-L.~Hsu}\affiliation{\instSydney} % 2299
  \author{Y.~Hu}\affiliation{\instIHEPChina} % 2227
  \author{K.~Huang}\affiliation{\instNTUTaiwan} % 2389
  \author{T.~Iijima}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2446
  \author{K.~Inami}\affiliation{\instNagoya} % 2323
  \author{G.~Inguglia}\affiliation{\instHEPHYVienna} % 2500
  \author{J.~Irakkathil~Jabbar}\affiliation{\instKarlsruhe} % 7343
  \author{A.~Ishikawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2281
  \author{R.~Itoh}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2487
  \author{M.~Iwasaki}\affiliation{\instOsakaCity} % 2360
  \author{Y.~Iwasaki}\affiliation{\instKEK} % 2229
  \author{S.~Iwata}\affiliation{\instTokyoMetropolitan} % 4323
  \author{P.~Jackson}\affiliation{\instAdelaide} % 2255
  \author{W.~W.~Jacobs}\affiliation{\instIndiana} % 2322
  \author{I.~Jaegle}\affiliation{\instFlorida} % 2539
  \author{D.~E.~Jaffe}\affiliation{\instBNL} % 3663
  \author{E.-J.~Jang}\affiliation{\instGyeongsang} % 6744
  \author{M.~Jeandron}\affiliation{\instMississippi} % 2806
  \author{H.~B.~Jeon}\affiliation{\instKyungpook} % 2170
  \author{S.~Jia}\affiliation{\instFudan} % 2457
  \author{Y.~Jin}\affiliation{\instTriesteINFN} % 2105
  \author{C.~Joo}\affiliation{\instIPMU} % 3525
  \author{K.~K.~Joo}\affiliation{\instChonnam} % 4224
  \author{I.~Kadenko}\affiliation{\instKyiv} % 3843
  \author{J.~Kahn}\affiliation{\instKarlsruhe} % 2448
  \author{H.~Kakuno}\affiliation{\instTokyoMetropolitan} % 2391
  \author{A.~B.~Kaliyar}\affiliation{\instTata} % 7344
  \author{J.~Kandra}\affiliation{\instPrague} % 2541
  \author{K.~H.~Kang}\affiliation{\instKyungpook} % 2283
  \author{P.~Kapusta}\affiliation{\instKrakow} % 6663
  \author{R.~Karl}\affiliation{\instDESY} % 10923
  \author{G.~Karyan}\affiliation{\instYerevan} % 2550
  \author{Y.~Kato}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2549
  \author{H.~Kawai}\affiliation{\instChiba} % 4344
  \author{T.~Kawasaki}\affiliation{\instKitasato} % 4363
  \author{T.~Keck}\affiliation{\instKarlsruhe} % 2300
  \author{C.~Ketter}\affiliation{\instHawaii} % 2236
  \author{H.~Kichimi}\affiliation{\instKEK} % 2233
  \author{C.~Kiesling}\affiliation{\instMPP} % 2168
  \author{B.~H.~Kim}\affiliation{\instSeoul} % 9743
  \author{C.-H.~Kim}\affiliation{\instHanyang} % 2358
  \author{D.~Y.~Kim}\affiliation{\instSoongsil} % 2315
  \author{H.~J.~Kim}\affiliation{\instKyungpook} % 4863
  \author{J.~B.~Kim}\affiliation{\instKorea} % 2408
  \author{K.-H.~Kim}\affiliation{\instYonsei} % 2118
  \author{K.~Kim}\affiliation{\instKorea} % 2409
  \author{S.-H.~Kim}\affiliation{\instSeoul} % 2428
  \author{Y.-K.~Kim}\affiliation{\instYonsei} % 2379
  \author{Y.~Kim}\affiliation{\instKorea} % 2403
  \author{T.~D.~Kimmel}\affiliation{\instVPI} % 2241
  \author{H.~Kindo}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2195
  \author{K.~Kinoshita}\affiliation{\instCincinnati} % 2318
  \author{B.~Kirby}\affiliation{\instBNL} % 5263
  \author{C.~Kleinwort}\affiliation{\instDESY} % 2499
  \author{B.~Knysh}\affiliation{\instIJCLab} % 8883
  \author{P.~Kody\v{s}}\affiliation{\instPrague} % 2407
  \author{T.~Koga}\affiliation{\instKEK} % 6963
  \author{S.~Kohani}\affiliation{\instHawaii} % 9143
  \author{I.~Komarov}\affiliation{\instDESY} % 2210
  \author{T.~Konno}\affiliation{\instKitasato} % 2490
  \author{S.~Korpar}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % 2475
% \author{E.~Kou}\affiliation{\instIJCLab} % 3765
  \author{N.~Kovalchuk}\affiliation{\instDESY} % 6964
  \author{T.~M.~G.~Kraetzschmar}\affiliation{\instMPP} % 7543
  \author{P.~Kri\v{z}an}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2474
  \author{R.~Kroeger}\affiliation{\instMississippi} % 2242
  \author{J.~F.~Krohn}\affiliation{\instMelbourne} % 2502
  \author{P.~Krokovny}\affiliation{\instBINP}\affiliation{\instNSU} % 2575
  \author{H.~Kr\"uger}\affiliation{\instBonn} % 2290
  \author{W.~Kuehn}\affiliation{\instGiessen} % 2534
  \author{T.~Kuhr}\affiliation{\instLMU} % 2486
  \author{J.~Kumar}\affiliation{\instCMU} % 6464
  \author{M.~Kumar}\affiliation{\instMNITJaipur} % 2744
  \author{R.~Kumar}\affiliation{\instPanjabPAU} % 2189
  \author{K.~Kumara}\affiliation{\instWayneState} % 2257
  \author{T.~Kumita}\affiliation{\instTokyoMetropolitan} % 4083
  \author{T.~Kunigo}\affiliation{\instKEK} % 10104
  \author{M.~K\"{u}nzel}\affiliation{\instDESY}\affiliation{\instLMU} % 2139
  \author{S.~Kurz}\affiliation{\instDESY} % 9363
  \author{A.~Kuzmin}\affiliation{\instBINP}\affiliation{\instNSU} % 2520
  \author{P.~Kvasni\v{c}ka}\affiliation{\instPrague} % 2184
  \author{Y.-J.~Kwon}\affiliation{\instYonsei} % 2231
  \author{S.~Lacaprara}\affiliation{\instPadovaINFN} % 2447
  \author{Y.-T.~Lai}\affiliation{\instIPMU} % 2066
  \author{C.~La~Licata}\affiliation{\instIPMU} % 2348
  \author{K.~Lalwani}\affiliation{\instMNITJaipur} % 2142
  \author{L.~Lanceri}\affiliation{\instTriesteINFN} % 2540
  \author{J.~S.~Lange}\affiliation{\instGiessen} % 2277
  \author{K.~Lautenbach}\affiliation{\instGiessen} % 2102
  \author{P.~J.~Laycock}\affiliation{\instBNL} % 7683
  \author{F.~R.~Le~Diberder}\affiliation{\instIJCLab} % 3267
  \author{I.-S.~Lee}\affiliation{\instHanyang} % 2422
  \author{S.~C.~Lee}\affiliation{\instKyungpook} % 2544
  \author{P.~Leitl}\affiliation{\instMPP} % 2414
  \author{D.~Levit}\affiliation{\instTUM} % 2507
  \author{P.~M.~Lewis}\affiliation{\instBonn} % 2582
  \author{C.~Li}\affiliation{\instLNNU} % 2325
  \author{C.-H.~Li}\affiliation{\instNTUTaiwan} % 2884  
  \author{L.~K.~Li}\affiliation{\instCincinnati} % 3263
  \author{S.~X.~Li}\affiliation{\instBeihang} % 2377
  \author{Y.~M.~Li}\affiliation{\instIHEPChina} % 2203
  \author{Y.~B.~Li}\affiliation{\instPeking} % 2573
  \author{J.~Libby}\affiliation{\instIITMadras} % 2262
  \author{K.~Lieret}\affiliation{\instLMU} % 2268
  \author{L.~Li~Gioi}\affiliation{\instMPP} % 2495
  \author{J.~Lin}\affiliation{\instNTUTaiwan} % 2401
  \author{Z.~Liptak}\affiliation{\instHawaii} % 3565
  \author{Q.~Y.~Liu}\affiliation{\instDESY} % 7045
  \author{Z.~A.~Liu}\affiliation{\instIHEPChina} % 3283
  \author{D.~Liventsev}\affiliation{\instWayneState}\affiliation{\instKEK} % 2578
  \author{S.~Longo}\affiliation{\instDESY} % 2396
  \author{A.~Loos}\affiliation{\instSCarolina} % 2356
  \author{P.~Lu}\affiliation{\instNTUTaiwan} % 2148
  \author{M.~Lubej}\affiliation{\instLjubljanaJSI} % 2513
  \author{T.~Lueck}\affiliation{\instLMU} % 2406
  \author{F.~Luetticke}\affiliation{\instBonn} % 2533
  \author{T.~Luo}\affiliation{\instFudan} % 3268
  \author{C.~MacQueen}\affiliation{\instMelbourne} % 2585
  \author{Y.~Maeda}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2427
  \author{M.~Maggiora}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 5343
  \author{S.~Maity}\affiliation{\instIITBhubaneswar} % 2985
  \author{R.~Manfredi}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 10303
  \author{E.~Manoni}\affiliation{\instPerugiaINFN} % 2305
  \author{S.~Marcello}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 4223
  \author{C.~Marinas}\affiliation{\instIFIC} % 2133
  \author{A.~Martini}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 2336
  \author{M.~Masuda}\affiliation{\instEri}\affiliation{\instRCNP} % 2238
  \author{T.~Matsuda}\affiliation{\instUOM} % 5543
  \author{K.~Matsuoka}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2316
  \author{D.~Matvienko}\affiliation{\instBINP}\affiliation{\instLPI}\affiliation{\instNSU} % 2351
  \author{J.~McNeil}\affiliation{\instFlorida} % 2382
  \author{F.~Meggendorfer}\affiliation{\instMPP} % 7103
  \author{J.~C.~Mei}\affiliation{\instFudan} % 7404
  \author{F.~Meier}\affiliation{\instDuke} % 3103
  \author{M.~Merola}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2456
  \author{F.~Metzner}\affiliation{\instKarlsruhe} % 2296
  \author{M.~Milesi}\affiliation{\instMelbourne} % 5443
  \author{C.~Miller}\affiliation{\instVictoria} % 2273
  \author{K.~Miyabayashi}\affiliation{\instNaraWu} % 2327
  \author{H.~Miyake}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2452
  \author{H.~Miyata}\affiliation{\instNiigata} % 2071
  \author{R.~Mizuk}\affiliation{\instLPI}\affiliation{\instHSE} % 2483
  \author{K.~Azmi}\affiliation{\instMalaya} % 2506
  \author{G.~B.~Mohanty}\affiliation{\instTata} % 2278
  \author{H.~Moon}\affiliation{\instKorea} % 2304
  \author{T.~Moon}\affiliation{\instSeoul} % 2397
  \author{J.~A.~Mora~Grimaldo}\affiliation{\instUTokyo} % 4403
  \author{A.~Morda}\affiliation{\instPadovaINFN} % 2503
  \author{T.~Morii}\affiliation{\instIPMU} % 3543
  \author{H.-G.~Moser}\affiliation{\instMPP} % 2120
  \author{M.~Mrvar}\affiliation{\instHEPHYVienna} % 2527
  \author{F.~Mueller}\affiliation{\instMPP} % 2240
  \author{F.~J.~M\"{u}ller}\affiliation{\instDESY} % 2123
  \author{Th.~Muller}\affiliation{\instKarlsruhe} % 2165
  \author{G.~Muroyama}\affiliation{\instNagoya} % 2093
  \author{C.~Murphy}\affiliation{\instIPMU} % 12403
  \author{R.~Mussa}\affiliation{\instTorinoINFN} % 2372
  \author{K.~Nakagiri}\affiliation{\instKEK} % 10103
  \author{I.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 3463
  \author{K.~R.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2417
  \author{E.~Nakano}\affiliation{\instOsakaCity} % 2554
  \author{M.~Nakao}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2498
  \author{H.~Nakayama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2232
  \author{H.~Nakazawa}\affiliation{\instNTUTaiwan} % 2335
  \author{T.~Nanut}\affiliation{\instLjubljanaJSI} % 2565
  \author{Z.~Natkaniec}\affiliation{\instKrakow} % 3923
  \author{A.~Natochii}\affiliation{\instHawaii} % 12063
  \author{M.~Nayak}\affiliation{\instTelAviv} % 2371
  \author{G.~Nazaryan}\affiliation{\instYerevan} % 9523
  \author{D.~Neverov}\affiliation{\instNagoya} % 2075
  \author{C.~Niebuhr}\affiliation{\instDESY} % 2477
  \author{M.~Niiyama}\affiliation{\instKSU} % 2063
  \author{J.~Ninkovic}\affiliation{\instMPGHLL} % 2386
  \author{N.~K.~Nisar}\affiliation{\instBNL} % 2522
  \author{S.~Nishida}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2571
  \author{K.~Nishimura}\affiliation{\instHawaii} % 3063
  \author{M.~Nishimura}\affiliation{\instKEK} % 7743
  \author{M.~H.~A.~Nouxman}\affiliation{\instMalaya} % 2470
  \author{B.~Oberhof}\affiliation{\instFrascati} % 2393
  \author{K.~Ogawa}\affiliation{\instNiigata} % 2430
  \author{S.~Ogawa}\affiliation{\instToho} % 6263
  \author{S.~L.~Olsen}\affiliation{\instGyeongsang} % 4563
  \author{Y.~Onishchuk}\affiliation{\instKyiv} % 2157
  \author{H.~Ono}\affiliation{\instNiigata} % 2160
  \author{Y.~Onuki}\affiliation{\instUTokyo} % 2331
  \author{P.~Oskin}\affiliation{\instLPI} % 9623
  \author{E.~R.~Oxford}\affiliation{\instCMU} % 6943
  \author{H.~Ozaki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2984
  \author{P.~Pakhlov}\affiliation{\instLPI}\affiliation{\instMEPhI} % 2221
  \author{G.~Pakhlova}\affiliation{\instHSE}\affiliation{\instLPI} % 2188
  \author{A.~Paladino}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2435
  \author{T.~Pang}\affiliation{\instPittsburgh} % 2114
  \author{A.~Panta}\affiliation{\instMississippi} % 7943
  \author{E.~Paoloni}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2488
  \author{S.~Pardi}\affiliation{\instNapoliINFN} % 2532
  \author{C.~Park}\affiliation{\instYonsei} % 2307
  \author{H.~Park}\affiliation{\instKyungpook} % 2284
  \author{S.-H.~Park}\affiliation{\instYonsei} % 2509
  \author{B.~Paschen}\affiliation{\instBonn} % 2159
  \author{A.~Passeri}\affiliation{\instRomaTreINFN} % 2116
  \author{A.~Pathak}\affiliation{\instLouisville} % 8723
  \author{S.~Patra}\affiliation{\instIISER} % 3123
  \author{S.~Paul}\affiliation{\instTUM} % 2131
  \author{T.~K.~Pedlar}\affiliation{\instLuther} % 2421
  \author{I.~Peruzzi}\affiliation{\instFrascati} % 2253
  \author{R.~Peschke}\affiliation{\instHawaii} % 7123
  \author{R.~Pestotnik}\affiliation{\instLjubljanaJSI} % 2476
  \author{M.~Piccolo}\affiliation{\instFrascati} % 2147
  \author{L.~E.~Piilonen}\affiliation{\instVPI} % 2346
  \author{P.~L.~M.~Podesta-Lerma}\affiliation{\instUAS} % 2266
  \author{G.~Polat}\affiliation{\instCPPM} % 9783
  \author{V.~Popov}\affiliation{\instHSE} % 2096
  \author{C.~Praz}\affiliation{\instDESY} % 2726
  \author{E.~Prencipe}\affiliation{\instJuelich} % 2219
  \author{M.~T.~Prim}\affiliation{\instBonn} % 2501
  \author{M.~V.~Purohit}\affiliation{\instOkinawa} % 2196
  \author{N.~Rad}\affiliation{\instDESY} % 11683
  \author{P.~Rados}\affiliation{\instDESY} % 7383
  \author{S.~Raiz}\affiliation{\instTriesteINFN} % 4564
  \author{R.~Rasheed}\affiliation{\instIPHC} % 3643
  \author{M.~Reif}\affiliation{\instMPP} % 8043
  \author{S.~Reiter}\affiliation{\instGiessen} % 2248
  \author{M.~Remnev}\affiliation{\instBINP}\affiliation{\instNSU} % 2785
  \author{P.~K.~Resmi}\affiliation{\instIITMadras} % 2588
  \author{I.~Ripp-Baudot}\affiliation{\instIPHC} % 2469
  \author{M.~Ritter}\affiliation{\instLMU} % 2580
  \author{M.~Ritzert}\affiliation{\instHeidelberg} % 2526
  \author{G.~Rizzo}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2579
  \author{L.~B.~Rizzuto}\affiliation{\instLjubljanaJSI} % 3746
  \author{S.~H.~Robertson}\affiliation{\instMcGill}\affiliation{\instIPP} % 2471
  \author{D.~Rodr\'{i}guez~P\'{e}rez}\affiliation{\instUAS} % 2176
  \author{J.~M.~Roney}\affiliation{\instVictoria}\affiliation{\instIPP} % 2244
  \author{C.~Rosenfeld}\affiliation{\instSCarolina} % 2082
  \author{A.~Rostomyan}\affiliation{\instDESY} % 2481
  \author{N.~Rout}\affiliation{\instIITMadras} % 2965
  \author{M.~Rozanska}\affiliation{\instKrakow} % 2205
  \author{G.~Russo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2388
  \author{D.~Sahoo}\affiliation{\instTata} % 2110
  \author{Y.~Sakai}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2175
  \author{D.~A.~Sanders}\affiliation{\instMississippi} % 2458
  \author{S.~Sandilya}\affiliation{\instCincinnati} % 2286
  \author{A.~Sangal}\affiliation{\instCincinnati} % 2384
  \author{L.~Santelj}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2185
  \author{P.~Sartori}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 4523
  \author{J.~Sasaki}\affiliation{\instUTokyo} % 4383
  \author{Y.~Sato}\affiliation{\instTohoku} % 5243
  \author{V.~Savinov}\affiliation{\instPittsburgh} % 2292
  \author{B.~Scavino}\affiliation{\instMainz} % 2518
  \author{M.~Schram}\affiliation{\instPNNL} % 2306
  \author{H.~Schreeck}\affiliation{\instGoettingen} % 2434
  \author{J.~Schueler}\affiliation{\instHawaii} % 2824
  \author{C.~Schwanda}\affiliation{\instHEPHYVienna} % 2108
  \author{A.~J.~Schwartz}\affiliation{\instCincinnati} % 2162
  \author{B.~Schwenker}\affiliation{\instGoettingen} % 2405
  \author{R.~M.~Seddon}\affiliation{\instMcGill} % 2314
  \author{Y.~Seino}\affiliation{\instNiigata} % 2517
  \author{A.~Selce}\affiliation{\instRomaUNIV}\affiliation{\instRomaINFN} % 9043
  \author{K.~Senyo}\affiliation{\instYamagata} % 2987
  \author{I.~S.~Seong}\affiliation{\instHawaii} % 2572
  \author{J.~Serrano}\affiliation{\instCPPM} % 12124
  \author{M.~E.~Sevior}\affiliation{\instMelbourne} % 2328
  \author{C.~Sfienti}\affiliation{\instMainz} % 2214
  \author{V.~Shebalin}\affiliation{\instHawaii} % 2339
  \author{C.~P.~Shen}\affiliation{\instBeihang} % 2464
  \author{H.~Shibuya}\affiliation{\instToho} % 2234
  \author{J.-G.~Shiu}\affiliation{\instNTUTaiwan} % 2412
  \author{B.~Shwartz}\affiliation{\instBINP}\affiliation{\instNSU} % 2122
  \author{A.~Sibidanov}\affiliation{\instVictoria} % 2419
  \author{F.~Simon}\affiliation{\instMPP} % 2164
  \author{J.~B.~Singh}\affiliation{\instPanjab} % 2903
  \author{S.~Skambraks}\affiliation{\instMPP} % 2394
  \author{K.~Smith}\affiliation{\instMelbourne} % 2243
  \author{R.~J.~Sobie}\affiliation{\instVictoria}\affiliation{\instIPP} % 2472
  \author{A.~Soffer}\affiliation{\instTelAviv} % 2217
  \author{A.~Sokolov}\affiliation{\instIHEPRussia} % 2521
  \author{Y.~Soloviev}\affiliation{\instDESY} % 2479
  \author{E.~Solovieva}\affiliation{\instLPI} % 2398
  \author{S.~Spataro}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2117
  \author{B.~Spruck}\affiliation{\instMainz} % 2493
  \author{M.~Stari\v{c}}\affiliation{\instLjubljanaJSI} % 2326
  \author{S.~Stefkova}\affiliation{\instDESY} % 8783
  \author{Z.~S.~Stottler}\affiliation{\instVPI} % 2267
  \author{R.~Stroili}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 2465
  \author{J.~Strube}\affiliation{\instPNNL} % 2451
  \author{J.~Stypula}\affiliation{\instKrakow} % 2368
  \author{M.~Sumihama}\affiliation{\instGifu}\affiliation{\instRCNP} % 4243
  \author{K.~Sumisawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2583
  \author{T.~Sumiyoshi}\affiliation{\instTokyoMetropolitan} % 4184
  \author{D.~J.~Summers}\affiliation{\instMississippi} % 7405
  \author{W.~Sutcliffe}\affiliation{\instBonn} % 3784
  \author{K.~Suzuki}\affiliation{\instNagoya} % 2445
  \author{S.~Y.~Suzuki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2496
  \author{H.~Svidras}\affiliation{\instDESY} % 11783
  \author{M.~Tabata}\affiliation{\instChiba} % 2986
  \author{M.~Takahashi}\affiliation{\instDESY} % 2467
  \author{M.~Takizawa}\affiliation{\instRIKENMSL}\affiliation{\instJPARC}\affiliation{\instSPU} % 2437
  \author{U.~Tamponi}\affiliation{\instTorinoINFN} % 2366
  \author{S.~Tanaka}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2530
  \author{K.~Tanida}\affiliation{\instJAEA} % 3803
  \author{H.~Tanigawa}\affiliation{\instUTokyo} % 2237
  \author{N.~Taniguchi}\affiliation{\instKEK} % 2285
  \author{Y.~Tao}\affiliation{\instFlorida} % 2362
  \author{P.~Taras}\affiliation{\instMontreal} % 2202
  \author{F.~Tenchini}\affiliation{\instDESY} % 2546
  \author{D.~Tonelli}\affiliation{\instTriesteINFN} % 4564
  \author{E.~Torassa}\affiliation{\instPadovaINFN} % 2556
  \author{K.~Trabelsi}\affiliation{\instIJCLab} % 2369
  \author{T.~Tsuboyama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2361
  \author{N.~Tsuzuki}\affiliation{\instNagoya} % 2352
  \author{M.~Uchida}\affiliation{\instTitech} % 2370
  \author{I.~Ueda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2519
  \author{S.~Uehara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2586
  \author{T.~Ueno}\affiliation{\instTohoku} % 4364
  \author{T.~Uglov}\affiliation{\instLPI}\affiliation{\instHSE} % 2252
  \author{K.~Unger}\affiliation{\instKarlsruhe} % 9463
  \author{Y.~Unno}\affiliation{\instHanyang} % 2420
  \author{S.~Uno}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2149
  \author{P.~Urquijo}\affiliation{\instMelbourne} % 2302
  \author{Y.~Ushiroda}\affiliation{\instKEK}\affiliation{\instSOKENDAI}\affiliation{\instUTokyo} % 2317
  \author{Y.~Usov}\affiliation{\instBINP}\affiliation{\instNSU} % 5003
  \author{S.~E.~Vahsen}\affiliation{\instHawaii} % 2251
  \author{R.~van~Tonder}\affiliation{\instBonn} % 2706
  \author{G.~S.~Varner}\affiliation{\instHawaii} % 2119
  \author{K.~E.~Varvell}\affiliation{\instSydney} % 2545
  \author{A.~Vinokurova}\affiliation{\instBINP}\affiliation{\instNSU} % 2289
  \author{L.~Vitale}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 2415
  \author{V.~Vorobyev}\affiliation{\instBINP}\affiliation{\instLPI}\affiliation{\instNSU} % 2298
  \author{A.~Vossen}\affiliation{\instDuke} % 2249
  \author{B.~Wach}\affiliation{\instMPP} % 2120  
  \author{E.~Waheed}\affiliation{\instKEK} % 2226
  \author{H.~M.~Wakeling}\affiliation{\instMcGill} % 3664
  \author{K.~Wan}\affiliation{\instUTokyo} % 2591
  \author{W.~Wan~Abdullah}\affiliation{\instMalaya} % 2280
  \author{B.~Wang}\affiliation{\instMPP} % 2569
  \author{C.~H.~Wang}\affiliation{\instNUUTaiwan} % 2224
  \author{M.-Z.~Wang}\affiliation{\instNTUTaiwan} % 2074
  \author{X.~L.~Wang}\affiliation{\instFudan} % 2076
  \author{A.~Warburton}\affiliation{\instMcGill} % 2347
  \author{M.~Watanabe}\affiliation{\instNiigata} % 2309
  \author{S.~Watanuki}\affiliation{\instIJCLab} % 6843
  \author{I.~Watson}\affiliation{\instUTokyo} % 2337
  \author{J.~Webb}\affiliation{\instMelbourne} % 2423
  \author{S.~Wehle}\affiliation{\instDESY} % 2489
  \author{M.~Welsch}\affiliation{\instBonn} % 7023
  \author{C.~Wessel}\affiliation{\instBonn} % 2100
  \author{J.~Wiechczynski}\affiliation{\instPisaINFN} % 2604
  \author{P.~Wieduwilt}\affiliation{\instGoettingen} % 2343
  \author{H.~Windel}\affiliation{\instMPP} % 2081
  \author{E.~Won}\affiliation{\instKorea} % 2410
  \author{L.~J.~Wu}\affiliation{\instIHEPChina} % 2704
  \author{X.~P.~Xu}\affiliation{\instSoochow} % 4923
  \author{B.~Yabsley}\affiliation{\instSydney} % 3645
  \author{S.~Yamada}\affiliation{\instKEK} % 2492
  \author{W.~Yan}\affiliation{\instUSTC} % 2094
  \author{S.~B.~Yang}\affiliation{\instKorea} % 2374
  \author{H.~Ye}\affiliation{\instDESY} % 2537
  \author{J.~Yelton}\affiliation{\instFlorida} % 2067
  \author{I.~Yeo}\affiliation{\instKISTI} % 2204
  \author{J.~H.~Yin}\affiliation{\instKorea} % 2365
  \author{M.~Yonenaga}\affiliation{\instTokyoMetropolitan} % 2411
  \author{Y.~M.~Yook}\affiliation{\instIHEPChina} % 2453
  \author{T.~Yoshinobu}\affiliation{\instNiigata} % 2429
  \author{C.~Z.~Yuan}\affiliation{\instIHEPChina} % 2088
  \author{G.~Yuan}\affiliation{\instUSTC} % 7243
  \author{W.~Yuan}\affiliation{\instPadovaINFN} % 2504
  \author{Y.~Yusa}\affiliation{\instNiigata} % 2357
  \author{L.~Zani}\affiliation{\instCPPM} % 2529
  \author{J.~Z.~Zhang}\affiliation{\instIHEPChina} % 2349
  \author{Y.~Zhang}\affiliation{\instUSTC} % 2607
  \author{Z.~Zhang}\affiliation{\instUSTC} % 5363
  \author{V.~Zhilich}\affiliation{\instBINP}\affiliation{\instNSU} % 4703
  \author{Q.~D.~Zhou}\affiliation{\instNagoya}\affiliation{\instNagoyaIAR} % 7323
  \author{X.~Y.~Zhou}\affiliation{\instBeihang} % 2380
  \author{V.~I.~Zhukova}\affiliation{\instLPI} % 2387
  \author{V.~Zhulanov}\affiliation{\instBINP}\affiliation{\instNSU} % 4983
  \author{A.~Zupanc}\affiliation{\instLjubljanaJSI} % 2543
\collaboration{Belle II Collaboration}


==> contents/CSVar.tex <==
\section{Classifier training variables}
\label{app:train}
To discriminate against such background, we use a binary boosted decision-tree classifier that combines nonlinearly 39 variables known to provide statistical discrimination between $B$-meson signals and continuum background and to be uncorrelated, or loosely correlated, with $M_{bc}$ and $\Delta E$. The variables are quantities associated to event topology (global and signal-only angular configurations).
In order to separate $q\bar{q}$ background and signal $B\bar{B}$ events, we use the binary boosted decision-tree classifier (\texttt{FBDT}), based on \texttt{basf2}, which combines information of 39 nonlinear variables. Those variables are loosely or uncorrelated with $m_{bc}$ and $\Delta E$, including event shape, flavor-tagger, vertex information and kinematic-fit quality : 
\begin{itemize}
 \item \texttt{R2} - ratio between the second and zeroth Fox-Wolfram moments,
 \item \texttt{cosTBTO} - cosine of angle between thrust axis of signal $B$ (reconstructed) and thrust axis of tag-side $B$, that is the rest of event (\texttt{ROE}),
 \item \texttt{cosTBz} - cosine of angle between thrust axis of signal $B$ and beam axis,
 \item \texttt{thrustOm} - magnitude of thrust of tag-side $B$~(\texttt{ROE}),
 \item \texttt{cosHelicityAngleMomentum} - cosine of angle between the $2$-body decay axis (or $3$-body decay plane) in $B$-frame and the momentum of the $B$ in lab-frame,
 \item \texttt{thrustAxisCosTheta} - cosine of the polar angle component of the thrust axis,
 \item \texttt{KSFWVariables(mm2)} - missing mass squared,
 \item 14 Kakuno-Super-Fox-Wolfram moments,
 \item 9 CLEO cones, using only the tag-side particles~(\texttt{ROE}), to reduce correlation  with $\Delta E$ and $m_{\it bc}$.
  \item \texttt{useCMSFrame(cosTheta)} - polar angle of the signal-$B$ candidate in the $\Upsilon(4S)$ frame.
  \item \texttt{KSFWVariables(et)} - transverse energy,
  \item \texttt{qpKinLepton} - charge of the tag-side track with highest probability of being a primary lepton multiplied by the respective probability,
    \item \texttt{qpKaon} - charge of the tag-side track with highest probability of being a \mbox{$b\to c\to s$} kaon multiplied by the respective probability,
    \item \texttt{qpSlowPion} - charge of the tag-side track with highest probability of being a slow pion from the decay of a primary $D^{*}$ multiplied by the respective probability, 
    \item \texttt{FBDT\_qrCombined} - combined flavor $q$ times dilution factor $r$,
    \item \texttt{DeltaZ} - spacial difference between signal and tag-side $B$-meson-decay vertices in beam direction,
    \item \texttt{DeltaZErr} - uncertainty on \texttt{DeltaZ},
    \item \texttt{chiProb} - $p$-value of signal $B$-meson-decay vertex fit.
\end{itemize}

==> contents/Rare.tex <==
\section{Decay channels in generic backgrounds}
\label{app:Rare}
Generic $B\bar{B}$ background are investigated with 300 $fb^{-1}$ MC, they are shown in Table~.\ref{tab:BB_Kpi_detail} and .\ref{tab:BB_pipi_detail}
\begin{table}[!ht]
\begin{center}
\begin{tabular}{l c c c c}
\hline \hline
\multirow{2}{2.5cm}{Rare Decay} & \multirow{2}{2.5cm}{Yields in 300 $\rm fb^{-1}$ MC} & \multirow{2}{2.5cm}{Yields per $\rm fb^{-1}$ MC} & \multirow{2}{2.5cm}{$\mathcal{B} [10^{-6}]$ in decay table} & \multirow{2}{2.5cm}{$\mathcal{B} [10^{-6}]$ in PDG}\\
 & & & & \\
\hline
\multirow{2}{3.5cm}{$B^0 \to K^+ \rho^-,$  $\rho^- \to \pi^- \pi^0$} & \multirow{2}{*}{172} & \multirow{2}{*}{0.6} & \multirow{2}{*}{8.4}& \multirow{2}{*}{$7.0 \pm 0.9$}\\
 & & & & \\
$B^0 \to \pi^+ \pi^- \pi^0$ & 70 & 0.2 & 24 & $< 7.2 \times 10^{-4}$\\
$B^+ \to \pi^+ \pi^0 \pi^0$ & 55 & 0.2 & 26 & $< 8.9 \times 10^{-4}$\\
\multirow{2}{3.5cm}{$B^0 \to K_{0}^* \pi^0,$  $K_{0}^* \to K^+ \pi^-$} & \multirow{2}{*}{53} & \multirow{2}{*}{0.2} & \multirow{2}{*}{2.4} & \multirow{2}{*}{$3.3 \pm 0.6$}\\ & & & & \\
$B^0 \to K^+ \pi^- \pi^0$ & 30 & 0.1 & 27.5 & $37.8 \pm 3.2$\\
\multirow{2}{3.5cm}{$B^+ \to K^{*+} \pi^0,$  $K^{*+} \to K^+ \pi^0$} & \multirow{2}{*}{28} & \multirow{2}{*}{0.1} & \multirow{2}{*}{2.3} & \multirow{2}{*}{$6.8 \pm 0.9$}\\ & & & & \\
\multirow{2}{3.5cm}{$B^+ \to \rho^+ \pi^0,$  $\rho^+ \to \pi^+ \pi^0$} & \multirow{2}{*}{27} & \multirow{2}{*}{0.1} & \multirow{2}{*}{10.9} & \multirow{2}{*}{$10.9 \pm 1.4$}\\ & & & & \\
%Other\tablefootnote[1]
Other & 250 & 0.8 &  & \\
\hline \hline
\end{tabular} 
\caption{Rare components in $B^+\to K^+\pi^0$ peaking background.}
\label{tab:BB_Kpi_detail}
\end{center}
\end{table}
%\tablefootnotetext[1]{Other in table means : Event with 1.bad reconstruction of $\pi^0$ 2.Can't trace MC-Truth information 3.Contribute yields less than 5$\%$.}
\begin{table}[!ht]
\begin{center}
\begin{tabular}{l c c c c}
\hline \hline
\multirow{2}{2.5cm}{Rare Decay} & \multirow{2}{2.5cm}{Yields in 300 $\rm fb^{-1}$ MC} & \multirow{2}{2.5cm}{Yields per $\rm fb^{-1}$ MC} & \multirow{2}{2.5cm}{$\mathcal{B} [10^{-6}]$ in decay table} & \multirow{2}{2.5cm}{$\mathcal{B} [10^{-6}]$ in PDG}\\
 & & & & \\
\hline
$B^0 \to \pi^+ \pi^- \pi^0$ & 492 & 1.6 & 24 & $< 7.2 \times 10^{-4}$\\
$B^+ \to \pi^+ \pi^0 \pi^0$ & 409 & 1.4 & 26 & $< 8.9 \times 10^{-4}$\\
\multirow{2}{3.5cm}{$B^+ \to \rho^+ \pi^0,$  $\rho^+ \to \pi^+ \pi^0$} & \multirow{2}{*}{56} & \multirow{2}{*}{0.2} & \multirow{2}{*}{10.9} & \multirow{2}{*}{$10.9 \pm 1.4$}\\ & & & & \\
\multirow{3}{3.5cm}{$B^0 \to \rho^+ \pi^- f_0,$  $\rho^+ \to \pi^+ \pi^0,$  $f_0 \to \pi^+ \pi^-$} & \multirow{3}{*}{36} & \multirow{3}{*}{0.1} & \multirow{3}{*}{5} & \multirow{3}{*}{}\\ & & & & \\ & & & & \\
\multirow{2}{3.5cm}{$B^+ \to f_0 \pi^+ \pi^0,$  $f_0 \to \pi^+ \pi^-$} & \multirow{2}{*}{30} & \multirow{2}{*}{0.1} & \multirow{2}{*}{5} & \multirow{2}{*}{}\\ & & & & \\
%Other\tablefootnote[1]
Other & 332 & 1.1 &  & \\
\hline \hline
\end{tabular} 
\caption{Rare components in $B^+\to \pi^+\pi^0$ peaking background.}
\label{tab:BB_pipi_detail}
\end{center}
\end{table}

==> contents/Systematic_Error.tex <==
\section{Systematic Uncertainties}
\label{sec:sys}
We consider several sources of systematic uncertainties. We assume the sources to be independent and add in quadrature the corresponding uncertainties. Table.~\ref{tab:tol_BR_sys} and ~\ref{tab:tol_acp_sys} summaries systematic uncertainties for the measurement of the branching fraction and CP asymmetry, respectively. Each contribution is detailed in the following.
\subsection{Tracking}
We assess a systematic uncertainty associated with possible data-simulation discrepancies in the reconstruction of charged particles~\cite{Tracking:2020}. The tracking efficiency in data agrees with the value observed in simulation within a $0.91\%$ uncertainty, which we (linearly) add as systematic uncertainty for each final-state charged particle.
\label{subsec:tracking}
\subsection{$\pi^0$ Selection}
We assess a systematic uncertainty associated with possible data-simulation discrepancies in the $\pi^0$ reconstruction and selection using the decays $B^0 \to D^{*-}(\to \bar{D}^0 (\to K^+\pi^-\pi^0)\pi^-) \pi^+$ and $B^0 \to D^{*-}(\to \bar{D}^0 (\to K^+\pi^-\pi^0)\pi^-) \pi^+$ where the selection of charged particle is identical and all distributions are weighted so as the $\pi^0$ momentum matches the $\pi^0$ momentum in charmless channels. We compare the yields obtained from fits to the $\Delta E$ distribution of reconstructed $B$ candidates and obtain an efficiency in data that agree with the value observed in simulation within a $13\%$ uncertainty, which is used as systematic uncertainty.
\label{subsec:pi0}
\subsection{Continuum suppression}
We evaluate data-MC discrepancies in the continuum-suppression distributions using the control channel $B^+ \to \bar{D}^0(\to K^+\pi^-\pi^0) \pi^+$. We find that the selection efficiency obtained in data and simulation agrees well, hence the statistical uncertainty on the ratio of data to MC efficiency is assigned as the systematic uncertainty.
\label{subsec:BDT_selection}
\subsection{$N_{B\bar{B}}$}
We assign a $1.4\%$ systematic uncertainty on the number of $B\bar{B}$ pairs, which includes the uncertainty on cross-section, integrated luminosity~\cite{Abudinen:2019osb} and potential shifts from the peak center-of-mass energy during the run periods.
\label{subsec:NBB}
\subsection{Fit components modeling}
\label{subsec:pdf}
Because we used empirical fit models for signal and feed-across, we assess a systematic uncertainty associated with the model choice. We use ensembles simplified simulated experiments, where the distribution for signal and background models are generated according to the default fitting model or to an alternative model. We fit the composition of all toy samples using the same likelihood as for the data and use the difference between the means of the branching fraction or CP asymmetry distributions to determine the systematic uncertainty of branching-fraction and CP asymmetry measurement.

For $B\bar{B}$ background, we use Kernel-Estimated PDFs to model the shape from simulation and some decay channels in our background are still not well-measured and studied. the shape will not be consistent with data. To estimated the systematic uncertainty from MC-data discrepancy in shape, we perform a alternative fit, where the fitting region is restricted to be $-0.12 < \Delta E < 0.3$ (GeV) and the number of $B\bar{B}$ background is fixed to be 0. We assign the difference on branching ratio and CP asymmetry as the systematic uncertainty.
\subsection{Model asymmetry}
\label{subsec:pdf_acp}
To estimate the asymmetry in fit models, we perform alternative fits, we allow asymmetries in fudge factor and mean shift for signal and feed-across and asymmetries in shape parameters for $q\bar{q}$ background. The variations in CP asymmetry results are quoted as the systematic uncertainties.
\subsection{Detector Bias}
We consider the uncertainty on the values of $\mathcal{A}_{det}$ (Table.~\ref{tab:ins_acp}) as systematic uncertainty due to instrumental asymmetry corrections in measurements of CP asymmetries. 
\label{subsec:dete}
\subsection{Summary}
\label{sec:Summary}
We summarize all of the systematic uncertainties in both branching fractions and CP asymmeries (See Table.~\ref{tab:tol_BR_sys}, ~\ref{tab:tol_acp_sys}). The total systematic error is the square root of the quadratic sum of all the terms.
\begin{table}[!ht]
\begin{center}
\begin{tabular}{l  c  c}
\hline\hline
Source & $B^+ \to K^+ \pi^0$ & $B^+ \to \pi^+ \pi^0$ \\
\hline
Tracking & $0.91\%$ & $0.91\%$ \\
$\pi^0$ efficiency & $13.00\%$ & $13.00\%$ \\
Continuum suppression & $2.90\%$ & $3.30\%$ \\
$N_{B\bar{B}}$ & $1.40\%$ & $1.40\%$ \\
Signal, feed-across model & $0.84\%$ & $1.37\%$ \\
$B\bar{B}$ background model & $0.40\%$ & $1.44\%$ \\
$q\bar{q}$ background model & $0.55\%$ & $2.49\%$ \\
\hline
Total & $13.47\%$ & $13.89\%$ \\
\hline\hline
\end{tabular}
\caption{Systematic uncertainties in branching fractions measurement}
\label{tab:tol_BR_sys}
\end{center}
\end{table}
\begin{table}[!ht]
\begin{center}
\begin{tabular}{l  c  c}
\hline\hline
Source & $B^+ \to K^+ \pi^0$ & $B^+ \to \pi^+ \pi^0$ \\
\hline
Detector bias & $0.019$ & $0.019$ \\
Signal, feed-across model & $0.008$ & $0.004$ \\
Background model & $0.014$ & $0.059$ \\
\hline
Total & $0.025$ & $0.062$ \\
\hline\hline
\end{tabular}
\caption{Systematic uncertainties in CP asymmetries measurement}
\label{tab:tol_acp_sys}
\end{center}
\end{table}

